An Einstein@home search for continuous gravitational waves from Cassiopeia A

We report the results of a directed search for continuous gravitational-wave emission in a broad frequency range (between 50 and 1000 Hz) from the central compact object of the supernova remnant Cassiopeia A (Cas A). The data comes from the sixth science run of LIGO and the search is performed on the volunteer distributed computing network Einstein@Home. We find no significant signal candidate, and set the most constraining upper limits to date on the gravitational-wave emission from Cas A, which beat the indirect age-based upper limit across the entire search range. At around 170 Hz (the most sensitive frequency range), we set 90% confidence upper limits on the gravitational wave amplitude $h_0$ of $\sim\!\!~2.9\times 10^{-25}$, roughly twice as constraining as the upper limits from previous searches on Cas A. The upper limits can also be expressed as constraints on the ellipticity of Cas A; with a few reasonable assumptions, we show that at gravitational-wave frequencies greater than 300~Hz, we can exclude an ellipticity of $\gtrsim\!\!~10^{-5}$.

==> table_ULs.tex <==
\begin{longtable}{|rr|ccc|}
\hline
\hline
\textbf{start}  & \textbf{stop}  &  $\mathbf{h_0^{90\%}}$  &  $\pm$  & $\mathbf{\Delta h_0^{90\%}}$ \\ 
\textbf{(Hz)}  & \textbf{(Hz)}  &  ($10^{-25}$)  & &  ($10^{-25}$) \\ 
\hline
\hline
\endhead
50.000	& 91.150	& 17.0	& $\pm$ & 1.4 \\
91.150	& 108.600	& 5.7	& $\pm$ & 0.5 \\
108.600	& 122.950	& 4.6	& $\pm$ & 0.4 \\
122.950	& 132.850	& 4.6	& $\pm$ & 0.4 \\
132.850	& 142.450	& 3.8	& $\pm$ & 0.3 \\
142.450	& 151.400	& 3.2	& $\pm$ & 0.3 \\
151.400	& 157.750	& 3.0	& $\pm$ & 0.2 \\
157.750	& 164.050	& 2.9	& $\pm$ & 0.2 \\
164.050	& 169.800	& 2.9	& $\pm$ & 0.2 \\
169.800	& 174.950	& 2.9	& $\pm$ & 0.2 \\
174.950	& 181.000	& 2.9	& $\pm$ & 0.2 \\
181.000	& 185.750	& 3.1	& $\pm$ & 0.3 \\
185.750	& 190.250	& 3.9	& $\pm$ & 0.3 \\
190.250	& 195.450	& 3.2	& $\pm$ & 0.3 \\
195.450	& 200.500	& 3.6	& $\pm$ & 0.3 \\
200.500	& 204.200	& 3.1	& $\pm$ & 0.3 \\
204.200	& 208.600	& 3.7	& $\pm$ & 0.3 \\
208.600	& 212.300	& 3.3	& $\pm$ & 0.3 \\
212.300	& 215.700	& 3.0	& $\pm$ & 0.2 \\
215.700	& 219.550	& 3.1	& $\pm$ & 0.3 \\
219.550	& 222.700	& 2.9	& $\pm$ & 0.2 \\
222.700	& 225.850	& 2.8	& $\pm$ & 0.2 \\
225.850	& 228.800	& 2.8	& $\pm$ & 0.2 \\
228.800	& 231.900	& 3.0	& $\pm$ & 0.2 \\
231.900	& 235.100	& 2.9	& $\pm$ & 0.2 \\
235.100	& 237.850	& 3.0	& $\pm$ & 0.2 \\
237.850	& 240.950	& 3.0	& $\pm$ & 0.2 \\
240.950	& 244.850	& 3.0	& $\pm$ & 0.2 \\
244.850	& 247.350	& 2.9	& $\pm$ & 0.2 \\
247.350	& 249.800	& 3.0	& $\pm$ & 0.2 \\
249.800	& 252.650	& 2.9	& $\pm$ & 0.2 \\
252.650	& 255.000	& 3.0	& $\pm$ & 0.2 \\
255.000	& 257.450	& 3.0	& $\pm$ & 0.2 \\
257.450	& 259.700	& 3.0	& $\pm$ & 0.2 \\
259.700	& 262.600	& 3.0	& $\pm$ & 0.2 \\
262.600	& 264.800	& 3.2	& $\pm$ & 0.3 \\
264.800	& 266.950	& 3.0	& $\pm$ & 0.2 \\
266.950	& 269.250	& 3.0	& $\pm$ & 0.2 \\
269.250	& 271.400	& 3.1	& $\pm$ & 0.3 \\
271.400	& 273.450	& 3.1	& $\pm$ & 0.3 \\
273.450	& 276.050	& 3.2	& $\pm$ & 0.3 \\
276.050	& 278.100	& 3.3	& $\pm$ & 0.3 \\
278.100	& 280.100	& 3.2	& $\pm$ & 0.3 \\
280.100	& 282.050	& 3.2	& $\pm$ & 0.3 \\
282.050	& 283.950	& 3.3	& $\pm$ & 0.3 \\
283.950	& 285.800	& 3.4	& $\pm$ & 0.3 \\
285.800	& 287.650	& 3.5	& $\pm$ & 0.3 \\
287.650	& 289.500	& 3.6	& $\pm$ & 0.3 \\
289.500	& 292.050	& 3.4	& $\pm$ & 0.3 \\
292.050	& 293.850	& 3.3	& $\pm$ & 0.3 \\
293.850	& 295.650	& 3.3	& $\pm$ & 0.3 \\
295.650	& 297.350	& 3.4	& $\pm$ & 0.3 \\
297.350	& 299.050	& 3.3	& $\pm$ & 0.3 \\
299.050	& 301.400	& 3.4	& $\pm$ & 0.3 \\
301.400	& 303.050	& 3.4	& $\pm$ & 0.3 \\
303.050	& 304.700	& 3.4	& $\pm$ & 0.3 \\
304.700	& 306.400	& 3.4	& $\pm$ & 0.3 \\
306.400	& 308.150	& 4.0	& $\pm$ & 0.3 \\
308.150	& 309.800	& 3.5	& $\pm$ & 0.3 \\
309.800	& 311.350	& 3.6	& $\pm$ & 0.3 \\
311.350	& 312.900	& 3.6	& $\pm$ & 0.3 \\
312.900	& 314.450	& 3.6	& $\pm$ & 0.3 \\
314.450	& 316.000	& 3.7	& $\pm$ & 0.3 \\
316.000	& 317.500	& 3.7	& $\pm$ & 0.3 \\
317.500	& 319.750	& 3.8	& $\pm$ & 0.3 \\
319.750	& 321.250	& 3.8	& $\pm$ & 0.3 \\
321.250	& 322.750	& 3.7	& $\pm$ & 0.3 \\
322.750	& 324.250	& 3.9	& $\pm$ & 0.3 \\
324.250	& 325.650	& 3.9	& $\pm$ & 0.3 \\
325.650	& 327.100	& 3.9	& $\pm$ & 0.3 \\
327.100	& 328.500	& 4.1	& $\pm$ & 0.3 \\
328.500	& 331.250	& 4.4	& $\pm$ & 0.4 \\
331.250	& 332.700	& 4.5	& $\pm$ & 0.4 \\
332.700	& 334.050	& 4.7	& $\pm$ & 0.4 \\
334.050	& 335.850	& 5.2	& $\pm$ & 0.4 \\
335.850	& 337.200	& 5.2	& $\pm$ & 0.4 \\
337.200	& 338.500	& 5.1	& $\pm$ & 0.4 \\
338.500	& 340.550	& 5.3	& $\pm$ & 0.4 \\
340.550	& 342.050	& 6.7	& $\pm$ & 0.5 \\
342.050	& 345.650	& 7.0	& $\pm$ & 0.6 \\
345.650	& 348.850	& 7.2	& $\pm$ & 0.6 \\
348.850	& 350.650	& 9.0	& $\pm$ & 0.7 \\
350.650	& 352.350	& 14.2	& $\pm$ & 1.2 \\
352.350	& 353.550	& 87.3	& $\pm$ & 7.2 \\
353.550	& 354.800	& 79.0	& $\pm$ & 6.5 \\
354.800	& 356.300	& 15.1	& $\pm$ & 1.2 \\
356.300	& 357.500	& 9.2	& $\pm$ & 0.8 \\
357.500	& 358.700	& 7.9	& $\pm$ & 0.6 \\
358.700	& 360.000	& 7.8	& $\pm$ & 0.6 \\
360.000	& 361.150	& 7.9	& $\pm$ & 0.7 \\
361.150	& 362.300	& 8.9	& $\pm$ & 0.7 \\
362.300	& 363.450	& 6.2	& $\pm$ & 0.5 \\
363.450	& 364.600	& 5.8	& $\pm$ & 0.5 \\
364.600	& 365.750	& 6.3	& $\pm$ & 0.5 \\
365.750	& 366.950	& 4.9	& $\pm$ & 0.4 \\
366.950	& 368.050	& 4.7	& $\pm$ & 0.4 \\
368.050	& 369.200	& 5.1	& $\pm$ & 0.4 \\
369.200	& 371.200	& 5.4	& $\pm$ & 0.4 \\
371.200	& 372.350	& 4.7	& $\pm$ & 0.4 \\
372.350	& 373.450	& 4.5	& $\pm$ & 0.4 \\
373.450	& 375.150	& 4.6	& $\pm$ & 0.4 \\
375.150	& 376.250	& 4.4	& $\pm$ & 0.4 \\
376.250	& 377.300	& 4.5	& $\pm$ & 0.4 \\
377.300	& 378.350	& 4.5	& $\pm$ & 0.4 \\
378.350	& 379.450	& 4.3	& $\pm$ & 0.3 \\
379.450	& 380.500	& 4.4	& $\pm$ & 0.4 \\
380.500	& 381.500	& 4.5	& $\pm$ & 0.4 \\
381.500	& 382.550	& 4.4	& $\pm$ & 0.4 \\
382.550	& 383.800	& 5.2	& $\pm$ & 0.4 \\
383.800	& 384.850	& 4.4	& $\pm$ & 0.4 \\
384.850	& 385.850	& 4.2	& $\pm$ & 0.3 \\
385.850	& 386.850	& 4.2	& $\pm$ & 0.3 \\
386.850	& 387.900	& 4.3	& $\pm$ & 0.4 \\
387.900	& 388.900	& 4.5	& $\pm$ & 0.4 \\
388.900	& 390.100	& 4.7	& $\pm$ & 0.4 \\
390.100	& 391.100	& 5.1	& $\pm$ & 0.4 \\
391.100	& 394.400	& 5.9	& $\pm$ & 0.5 \\
394.400	& 395.450	& 4.7	& $\pm$ & 0.4 \\
395.450	& 397.550	& 4.4	& $\pm$ & 0.4 \\
397.550	& 398.500	& 4.6	& $\pm$ & 0.4 \\
398.500	& 399.650	& 4.3	& $\pm$ & 0.4 \\
399.650	& 401.900	& 4.5	& $\pm$ & 0.4 \\
401.900	& 402.950	& 4.3	& $\pm$ & 0.4 \\
402.950	& 404.900	& 4.3	& $\pm$ & 0.3 \\
404.900	& 405.800	& 4.4	& $\pm$ & 0.4 \\
405.800	& 406.750	& 4.2	& $\pm$ & 0.3 \\
406.750	& 407.800	& 4.4	& $\pm$ & 0.4 \\
407.800	& 408.750	& 4.2	& $\pm$ & 0.3 \\
408.750	& 409.750	& 4.3	& $\pm$ & 0.4 \\
409.750	& 410.650	& 4.2	& $\pm$ & 0.3 \\
410.650	& 411.550	& 4.2	& $\pm$ & 0.3 \\
411.550	& 412.550	& 4.3	& $\pm$ & 0.3 \\
412.550	& 414.150	& 4.1	& $\pm$ & 0.3 \\
414.150	& 415.050	& 4.2	& $\pm$ & 0.3 \\
415.050	& 415.900	& 4.2	& $\pm$ & 0.3 \\
415.900	& 417.900	& 4.2	& $\pm$ & 0.3 \\
417.900	& 418.850	& 4.3	& $\pm$ & 0.3 \\
418.850	& 419.700	& 4.4	& $\pm$ & 0.4 \\
419.700	& 420.600	& 4.3	& $\pm$ & 0.4 \\
420.600	& 421.450	& 4.3	& $\pm$ & 0.3 \\
421.450	& 422.300	& 4.2	& $\pm$ & 0.3 \\
422.300	& 423.250	& 4.3	& $\pm$ & 0.4 \\
423.250	& 424.100	& 4.3	& $\pm$ & 0.4 \\
424.100	& 424.950	& 5.0	& $\pm$ & 0.4 \\
424.950	& 425.750	& 4.5	& $\pm$ & 0.4 \\
425.750	& 426.600	& 4.4	& $\pm$ & 0.4 \\
426.600	& 427.450	& 4.6	& $\pm$ & 0.4 \\
427.450	& 428.250	& 4.6	& $\pm$ & 0.4 \\
428.250	& 429.100	& 4.4	& $\pm$ & 0.4 \\
429.100	& 430.500	& 4.6	& $\pm$ & 0.4 \\
430.500	& 431.350	& 5.0	& $\pm$ & 0.4 \\
431.350	& 432.150	& 5.1	& $\pm$ & 0.4 \\
432.150	& 432.950	& 5.2	& $\pm$ & 0.4 \\
432.950	& 433.750	& 5.8	& $\pm$ & 0.5 \\
433.750	& 435.300	& 5.9	& $\pm$ & 0.5 \\
435.300	& 436.100	& 5.2	& $\pm$ & 0.4 \\
436.100	& 436.850	& 5.8	& $\pm$ & 0.5 \\
436.850	& 437.650	& 5.4	& $\pm$ & 0.4 \\
437.650	& 438.450	& 4.8	& $\pm$ & 0.4 \\
438.450	& 439.250	& 4.5	& $\pm$ & 0.4 \\
439.250	& 440.600	& 4.5	& $\pm$ & 0.4 \\
440.600	& 441.450	& 4.4	& $\pm$ & 0.4 \\
441.450	& 442.250	& 4.5	& $\pm$ & 0.4 \\
442.250	& 443.000	& 4.4	& $\pm$ & 0.4 \\
443.000	& 443.800	& 4.4	& $\pm$ & 0.4 \\
443.800	& 444.800	& 4.5	& $\pm$ & 0.4 \\
444.800	& 445.600	& 4.5	& $\pm$ & 0.4 \\
445.600	& 446.350	& 4.5	& $\pm$ & 0.4 \\
446.350	& 447.100	& 4.5	& $\pm$ & 0.4 \\
447.100	& 447.850	& 4.4	& $\pm$ & 0.4 \\
447.850	& 448.600	& 4.4	& $\pm$ & 0.4 \\
448.600	& 449.350	& 4.4	& $\pm$ & 0.4 \\
449.350	& 450.100	& 4.4	& $\pm$ & 0.4 \\
450.100	& 450.850	& 4.4	& $\pm$ & 0.4 \\
450.850	& 452.000	& 4.6	& $\pm$ & 0.4 \\
452.000	& 452.750	& 4.6	& $\pm$ & 0.4 \\
452.750	& 453.500	& 4.6	& $\pm$ & 0.4 \\
453.500	& 454.250	& 4.7	& $\pm$ & 0.4 \\
454.250	& 455.050	& 4.6	& $\pm$ & 0.4 \\
455.050	& 455.800	& 4.6	& $\pm$ & 0.4 \\
455.800	& 456.550	& 4.8	& $\pm$ & 0.4 \\
456.550	& 457.250	& 4.7	& $\pm$ & 0.4 \\
457.250	& 458.100	& 4.7	& $\pm$ & 0.4 \\
458.100	& 458.800	& 4.7	& $\pm$ & 0.4 \\
458.800	& 459.550	& 4.9	& $\pm$ & 0.4 \\
459.550	& 460.250	& 5.0	& $\pm$ & 0.4 \\
460.250	& 461.200	& 4.8	& $\pm$ & 0.4 \\
461.200	& 461.950	& 4.8	& $\pm$ & 0.4 \\
461.950	& 462.650	& 4.6	& $\pm$ & 0.4 \\
462.650	& 463.350	& 4.5	& $\pm$ & 0.4 \\
463.350	& 464.050	& 4.6	& $\pm$ & 0.4 \\
464.050	& 464.750	& 4.5	& $\pm$ & 0.4 \\
464.750	& 465.450	& 4.5	& $\pm$ & 0.4 \\
465.450	& 466.150	& 4.7	& $\pm$ & 0.4 \\
466.150	& 466.850	& 4.6	& $\pm$ & 0.4 \\
466.850	& 467.550	& 4.6	& $\pm$ & 0.4 \\
467.550	& 468.800	& 4.7	& $\pm$ & 0.4 \\
468.800	& 469.500	& 4.7	& $\pm$ & 0.4 \\
469.500	& 470.150	& 4.7	& $\pm$ & 0.4 \\
470.150	& 470.850	& 5.0	& $\pm$ & 0.4 \\
470.850	& 471.550	& 5.2	& $\pm$ & 0.4 \\
471.550	& 472.250	& 5.0	& $\pm$ & 0.4 \\
472.250	& 472.950	& 5.0	& $\pm$ & 0.4 \\
472.950	& 473.650	& 5.0	& $\pm$ & 0.4 \\
473.650	& 474.300	& 4.8	& $\pm$ & 0.4 \\
474.300	& 475.000	& 4.9	& $\pm$ & 0.4 \\
475.000	& 475.650	& 5.0	& $\pm$ & 0.4 \\
475.650	& 476.350	& 5.1	& $\pm$ & 0.4 \\
476.350	& 477.000	& 5.2	& $\pm$ & 0.4 \\
477.000	& 477.650	& 4.9	& $\pm$ & 0.4 \\
477.650	& 478.350	& 5.1	& $\pm$ & 0.4 \\
478.350	& 479.000	& 5.0	& $\pm$ & 0.4 \\
479.000	& 479.650	& 5.0	& $\pm$ & 0.4 \\
479.650	& 480.300	& 5.0	& $\pm$ & 0.4 \\
480.300	& 480.950	& 5.1	& $\pm$ & 0.4 \\
480.950	& 481.650	& 4.9	& $\pm$ & 0.4 \\
481.650	& 482.900	& 4.9	& $\pm$ & 0.4 \\
482.900	& 483.550	& 5.0	& $\pm$ & 0.4 \\
483.550	& 484.200	& 4.8	& $\pm$ & 0.4 \\
484.200	& 484.850	& 4.9	& $\pm$ & 0.4 \\
484.850	& 485.450	& 5.8	& $\pm$ & 0.5 \\
485.450	& 487.150	& 5.0	& $\pm$ & 0.4 \\
487.150	& 487.800	& 4.9	& $\pm$ & 0.4 \\
487.800	& 488.450	& 5.1	& $\pm$ & 0.4 \\
488.450	& 489.100	& 4.9	& $\pm$ & 0.4 \\
489.100	& 489.700	& 4.9	& $\pm$ & 0.4 \\
489.700	& 490.350	& 4.9	& $\pm$ & 0.4 \\
490.350	& 491.050	& 4.9	& $\pm$ & 0.4 \\
491.050	& 491.650	& 4.8	& $\pm$ & 0.4 \\
491.650	& 492.300	& 4.9	& $\pm$ & 0.4 \\
492.300	& 492.900	& 4.9	& $\pm$ & 0.4 \\
492.900	& 493.550	& 4.9	& $\pm$ & 0.4 \\
493.550	& 494.150	& 5.0	& $\pm$ & 0.4 \\
494.150	& 494.800	& 5.3	& $\pm$ & 0.4 \\
494.800	& 495.400	& 5.3	& $\pm$ & 0.4 \\
495.400	& 496.200	& 5.1	& $\pm$ & 0.4 \\
496.200	& 496.850	& 5.3	& $\pm$ & 0.4 \\
496.850	& 497.450	& 5.3	& $\pm$ & 0.4 \\
497.450	& 498.050	& 5.4	& $\pm$ & 0.4 \\
498.050	& 498.650	& 5.9	& $\pm$ & 0.5 \\
498.650	& 499.300	& 6.3	& $\pm$ & 0.5 \\
499.300	& 499.900	& 6.0	& $\pm$ & 0.5 \\
499.900	& 500.500	& 5.8	& $\pm$ & 0.5 \\
500.500	& 501.100	& 5.2	& $\pm$ & 0.4 \\
501.100	& 501.700	& 5.2	& $\pm$ & 0.4 \\
501.700	& 502.300	& 5.3	& $\pm$ & 0.4 \\
502.300	& 502.900	& 5.2	& $\pm$ & 0.4 \\
502.900	& 503.500	& 5.0	& $\pm$ & 0.4 \\
503.500	& 504.100	& 5.0	& $\pm$ & 0.4 \\
504.100	& 504.700	& 5.2	& $\pm$ & 0.4 \\
504.700	& 505.300	& 5.0	& $\pm$ & 0.4 \\
505.300	& 505.900	& 4.9	& $\pm$ & 0.4 \\
505.900	& 506.500	& 4.9	& $\pm$ & 0.4 \\
506.500	& 507.100	& 4.9	& $\pm$ & 0.4 \\
507.100	& 507.650	& 5.0	& $\pm$ & 0.4 \\
507.650	& 508.250	& 4.9	& $\pm$ & 0.4 \\
508.250	& 508.850	& 5.0	& $\pm$ & 0.4 \\
508.850	& 509.450	& 5.0	& $\pm$ & 0.4 \\
509.450	& 510.000	& 5.1	& $\pm$ & 0.4 \\
510.000	& 510.600	& 5.0	& $\pm$ & 0.4 \\
510.600	& 511.200	& 5.0	& $\pm$ & 0.4 \\
511.200	& 511.750	& 4.9	& $\pm$ & 0.4 \\
511.750	& 512.450	& 4.9	& $\pm$ & 0.4 \\
512.450	& 513.000	& 4.9	& $\pm$ & 0.4 \\
513.000	& 513.600	& 4.9	& $\pm$ & 0.4 \\
513.600	& 514.200	& 5.0	& $\pm$ & 0.4 \\
514.200	& 514.750	& 5.0	& $\pm$ & 0.4 \\
514.750	& 515.300	& 5.0	& $\pm$ & 0.4 \\
515.300	& 515.900	& 5.0	& $\pm$ & 0.4 \\
515.900	& 516.500	& 5.0	& $\pm$ & 0.4 \\
516.500	& 517.100	& 5.1	& $\pm$ & 0.4 \\
517.100	& 517.650	& 5.0	& $\pm$ & 0.4 \\
517.650	& 518.200	& 5.0	& $\pm$ & 0.4 \\
518.200	& 518.850	& 5.1	& $\pm$ & 0.4 \\
518.850	& 519.400	& 5.3	& $\pm$ & 0.4 \\
519.400	& 519.950	& 5.1	& $\pm$ & 0.4 \\
519.950	& 520.500	& 5.0	& $\pm$ & 0.4 \\
520.500	& 521.100	& 5.0	& $\pm$ & 0.4 \\
521.100	& 521.650	& 5.1	& $\pm$ & 0.4 \\
521.650	& 522.200	& 5.1	& $\pm$ & 0.4 \\
522.200	& 522.750	& 5.1	& $\pm$ & 0.4 \\
522.750	& 523.300	& 5.1	& $\pm$ & 0.4 \\
523.300	& 524.700	& 5.1	& $\pm$ & 0.4 \\
524.700	& 525.250	& 5.1	& $\pm$ & 0.4 \\
525.250	& 525.800	& 5.1	& $\pm$ & 0.4 \\
525.800	& 526.350	& 5.1	& $\pm$ & 0.4 \\
526.350	& 526.900	& 5.2	& $\pm$ & 0.4 \\
526.900	& 527.450	& 5.2	& $\pm$ & 0.4 \\
527.450	& 528.000	& 5.3	& $\pm$ & 0.4 \\
528.000	& 528.550	& 5.5	& $\pm$ & 0.4 \\
528.550	& 529.100	& 5.8	& $\pm$ & 0.5 \\
529.100	& 529.650	& 5.5	& $\pm$ & 0.4 \\
529.650	& 530.150	& 5.4	& $\pm$ & 0.4 \\
530.150	& 530.700	& 5.4	& $\pm$ & 0.5 \\
530.700	& 531.250	& 5.3	& $\pm$ & 0.4 \\
531.250	& 531.800	& 5.2	& $\pm$ & 0.4 \\
531.800	& 532.400	& 5.2	& $\pm$ & 0.4 \\
532.400	& 532.900	& 5.2	& $\pm$ & 0.4 \\
532.900	& 533.450	& 5.2	& $\pm$ & 0.4 \\
533.450	& 534.000	& 5.2	& $\pm$ & 0.4 \\
534.000	& 534.500	& 5.2	& $\pm$ & 0.4 \\
534.500	& 535.050	& 5.3	& $\pm$ & 0.4 \\
535.050	& 535.600	& 5.2	& $\pm$ & 0.4 \\
535.600	& 536.100	& 5.3	& $\pm$ & 0.4 \\
536.100	& 536.650	& 5.3	& $\pm$ & 0.4 \\
536.650	& 537.150	& 5.2	& $\pm$ & 0.4 \\
537.150	& 537.700	& 5.3	& $\pm$ & 0.4 \\
537.700	& 538.200	& 5.3	& $\pm$ & 0.4 \\
538.200	& 538.750	& 5.2	& $\pm$ & 0.4 \\
538.750	& 539.250	& 5.2	& $\pm$ & 0.4 \\
539.250	& 539.800	& 5.2	& $\pm$ & 0.4 \\
539.800	& 540.300	& 5.2	& $\pm$ & 0.4 \\
540.300	& 540.800	& 5.2	& $\pm$ & 0.4 \\
540.800	& 541.350	& 5.2	& $\pm$ & 0.4 \\
541.350	& 541.850	& 5.2	& $\pm$ & 0.4 \\
541.850	& 542.400	& 5.3	& $\pm$ & 0.4 \\
542.400	& 542.900	& 5.2	& $\pm$ & 0.4 \\
542.900	& 543.400	& 5.2	& $\pm$ & 0.4 \\
543.400	& 543.900	& 5.5	& $\pm$ & 0.5 \\
543.900	& 544.450	& 5.7	& $\pm$ & 0.5 \\
544.450	& 544.950	& 5.2	& $\pm$ & 0.4 \\
544.950	& 545.450	& 5.2	& $\pm$ & 0.4 \\
545.450	& 546.550	& 5.2	& $\pm$ & 0.4 \\
546.550	& 547.100	& 5.3	& $\pm$ & 0.4 \\
547.100	& 547.600	& 5.2	& $\pm$ & 0.4 \\
547.600	& 548.100	& 5.2	& $\pm$ & 0.4 \\
548.100	& 548.600	& 5.2	& $\pm$ & 0.4 \\
548.600	& 549.100	& 5.4	& $\pm$ & 0.4 \\
549.100	& 549.600	& 5.2	& $\pm$ & 0.4 \\
549.600	& 550.100	& 5.2	& $\pm$ & 0.4 \\
550.100	& 550.600	& 5.3	& $\pm$ & 0.4 \\
550.600	& 552.600	& 5.3	& $\pm$ & 0.4 \\
552.600	& 553.100	& 5.3	& $\pm$ & 0.4 \\
553.100	& 553.600	& 5.3	& $\pm$ & 0.4 \\
553.600	& 554.100	& 5.3	& $\pm$ & 0.4 \\
554.100	& 554.600	& 5.3	& $\pm$ & 0.4 \\
554.600	& 555.100	& 5.3	& $\pm$ & 0.4 \\
555.100	& 555.550	& 5.3	& $\pm$ & 0.4 \\
555.550	& 556.050	& 5.4	& $\pm$ & 0.5 \\
556.050	& 556.550	& 5.5	& $\pm$ & 0.5 \\
556.550	& 557.050	& 5.3	& $\pm$ & 0.4 \\
557.050	& 557.550	& 5.3	& $\pm$ & 0.4 \\
557.550	& 558.050	& 5.3	& $\pm$ & 0.4 \\
558.050	& 558.500	& 5.3	& $\pm$ & 0.4 \\
558.500	& 559.000	& 5.4	& $\pm$ & 0.4 \\
559.000	& 559.500	& 5.3	& $\pm$ & 0.4 \\
559.500	& 559.950	& 5.4	& $\pm$ & 0.4 \\
559.950	& 560.450	& 5.4	& $\pm$ & 0.4 \\
560.450	& 560.950	& 5.5	& $\pm$ & 0.4 \\
560.950	& 561.400	& 5.4	& $\pm$ & 0.4 \\
561.400	& 561.900	& 5.4	& $\pm$ & 0.4 \\
561.900	& 562.450	& 5.4	& $\pm$ & 0.5 \\
562.450	& 562.900	& 5.4	& $\pm$ & 0.4 \\
562.900	& 563.400	& 5.4	& $\pm$ & 0.4 \\
563.400	& 564.650	& 5.4	& $\pm$ & 0.4 \\
564.650	& 565.150	& 5.4	& $\pm$ & 0.4 \\
565.150	& 565.600	& 5.5	& $\pm$ & 0.4 \\
565.600	& 566.650	& 5.4	& $\pm$ & 0.4 \\
566.650	& 567.100	& 5.5	& $\pm$ & 0.4 \\
567.100	& 568.750	& 5.6	& $\pm$ & 0.5 \\
568.750	& 569.200	& 5.4	& $\pm$ & 0.4 \\
569.200	& 569.700	& 5.4	& $\pm$ & 0.4 \\
569.700	& 570.250	& 5.5	& $\pm$ & 0.4 \\
570.250	& 570.700	& 5.4	& $\pm$ & 0.4 \\
570.700	& 571.200	& 5.4	& $\pm$ & 0.4 \\
571.200	& 571.650	& 5.5	& $\pm$ & 0.4 \\
571.650	& 572.100	& 5.4	& $\pm$ & 0.4 \\
572.100	& 572.550	& 5.5	& $\pm$ & 0.4 \\
572.550	& 573.050	& 5.5	& $\pm$ & 0.4 \\
573.050	& 573.500	& 5.5	& $\pm$ & 0.4 \\
573.500	& 573.950	& 5.4	& $\pm$ & 0.4 \\
573.950	& 574.400	& 5.6	& $\pm$ & 0.5 \\
574.400	& 574.900	& 5.6	& $\pm$ & 0.5 \\
574.900	& 575.500	& 5.4	& $\pm$ & 0.4 \\
575.500	& 575.950	& 5.5	& $\pm$ & 0.4 \\
575.950	& 576.400	& 5.5	& $\pm$ & 0.5 \\
576.400	& 576.850	& 5.6	& $\pm$ & 0.5 \\
576.850	& 577.300	& 5.8	& $\pm$ & 0.5 \\
577.300	& 577.750	& 5.5	& $\pm$ & 0.5 \\
577.750	& 578.250	& 5.5	& $\pm$ & 0.5 \\
578.250	& 578.700	& 5.6	& $\pm$ & 0.5 \\
578.700	& 579.150	& 5.7	& $\pm$ & 0.5 \\
579.150	& 580.850	& 5.7	& $\pm$ & 0.5 \\
580.850	& 581.300	& 5.8	& $\pm$ & 0.5 \\
581.300	& 581.750	& 5.9	& $\pm$ & 0.5 \\
581.750	& 582.200	& 6.1	& $\pm$ & 0.5 \\
582.200	& 582.650	& 6.3	& $\pm$ & 0.5 \\
582.650	& 583.100	& 6.9	& $\pm$ & 0.6 \\
583.100	& 583.550	& 7.5	& $\pm$ & 0.6 \\
583.550	& 584.000	& 6.6	& $\pm$ & 0.5 \\
584.000	& 584.400	& 6.4	& $\pm$ & 0.5 \\
584.400	& 584.850	& 5.8	& $\pm$ & 0.5 \\
584.850	& 585.300	& 5.9	& $\pm$ & 0.5 \\
585.300	& 585.750	& 5.8	& $\pm$ & 0.5 \\
585.750	& 586.200	& 5.8	& $\pm$ & 0.5 \\
586.200	& 586.650	& 5.7	& $\pm$ & 0.5 \\
586.650	& 587.100	& 5.7	& $\pm$ & 0.5 \\
587.100	& 587.500	& 5.7	& $\pm$ & 0.5 \\
587.500	& 587.950	& 5.8	& $\pm$ & 0.5 \\
587.950	& 588.400	& 5.8	& $\pm$ & 0.5 \\
588.400	& 588.850	& 5.9	& $\pm$ & 0.5 \\
588.850	& 589.250	& 5.9	& $\pm$ & 0.5 \\
589.250	& 589.750	& 6.1	& $\pm$ & 0.5 \\
589.750	& 590.200	& 5.8	& $\pm$ & 0.5 \\
590.200	& 590.650	& 5.8	& $\pm$ & 0.5 \\
590.650	& 591.050	& 5.8	& $\pm$ & 0.5 \\
591.050	& 591.500	& 6.2	& $\pm$ & 0.5 \\
591.500	& 591.950	& 6.4	& $\pm$ & 0.5 \\
591.950	& 592.350	& 6.3	& $\pm$ & 0.5 \\
592.350	& 592.800	& 6.2	& $\pm$ & 0.5 \\
592.800	& 593.250	& 6.1	& $\pm$ & 0.5 \\
593.250	& 593.650	& 6.2	& $\pm$ & 0.5 \\
593.650	& 594.100	& 6.1	& $\pm$ & 0.5 \\
594.100	& 594.550	& 6.3	& $\pm$ & 0.5 \\
594.550	& 594.950	& 6.2	& $\pm$ & 0.5 \\
594.950	& 595.400	& 6.1	& $\pm$ & 0.5 \\
595.400	& 595.800	& 5.9	& $\pm$ & 0.5 \\
595.800	& 596.250	& 5.8	& $\pm$ & 0.5 \\
596.250	& 596.650	& 5.9	& $\pm$ & 0.5 \\
596.650	& 597.100	& 5.9	& $\pm$ & 0.5 \\
597.100	& 597.500	& 5.8	& $\pm$ & 0.5 \\
597.500	& 597.950	& 5.8	& $\pm$ & 0.5 \\
597.950	& 598.350	& 5.9	& $\pm$ & 0.5 \\
598.350	& 598.800	& 5.7	& $\pm$ & 0.5 \\
598.800	& 599.200	& 5.8	& $\pm$ & 0.5 \\
599.200	& 599.650	& 5.8	& $\pm$ & 0.5 \\
599.650	& 600.050	& 5.9	& $\pm$ & 0.5 \\
600.050	& 600.500	& 5.8	& $\pm$ & 0.5 \\
600.500	& 600.900	& 5.8	& $\pm$ & 0.5 \\
600.900	& 601.400	& 6.1	& $\pm$ & 0.5 \\
601.400	& 601.800	& 5.9	& $\pm$ & 0.5 \\
601.800	& 602.200	& 5.9	& $\pm$ & 0.5 \\
602.200	& 602.650	& 6.0	& $\pm$ & 0.5 \\
602.650	& 603.050	& 6.5	& $\pm$ & 0.5 \\
603.050	& 603.450	& 7.0	& $\pm$ & 0.6 \\
603.450	& 603.900	& 6.1	& $\pm$ & 0.5 \\
603.900	& 604.300	& 6.1	& $\pm$ & 0.5 \\
604.300	& 604.700	& 5.9	& $\pm$ & 0.5 \\
604.700	& 605.150	& 5.9	& $\pm$ & 0.5 \\
605.150	& 605.550	& 6.0	& $\pm$ & 0.5 \\
605.550	& 605.950	& 6.1	& $\pm$ & 0.5 \\
605.950	& 606.400	& 5.9	& $\pm$ & 0.5 \\
606.400	& 606.800	& 5.8	& $\pm$ & 0.5 \\
606.800	& 607.200	& 6.0	& $\pm$ & 0.5 \\
607.200	& 608.500	& 5.9	& $\pm$ & 0.5 \\
608.500	& 608.950	& 5.9	& $\pm$ & 0.5 \\
608.950	& 609.350	& 5.9	& $\pm$ & 0.5 \\
609.350	& 609.750	& 5.9	& $\pm$ & 0.5 \\
609.750	& 610.150	& 6.0	& $\pm$ & 0.5 \\
610.150	& 610.550	& 5.9	& $\pm$ & 0.5 \\
610.550	& 610.950	& 5.9	& $\pm$ & 0.5 \\
610.950	& 611.400	& 6.0	& $\pm$ & 0.5 \\
611.400	& 611.800	& 6.2	& $\pm$ & 0.5 \\
611.800	& 612.200	& 6.3	& $\pm$ & 0.5 \\
612.200	& 612.600	& 6.1	& $\pm$ & 0.5 \\
612.600	& 613.000	& 6.4	& $\pm$ & 0.5 \\
613.000	& 613.400	& 6.2	& $\pm$ & 0.5 \\
613.400	& 613.800	& 6.3	& $\pm$ & 0.5 \\
613.800	& 614.200	& 6.2	& $\pm$ & 0.5 \\
614.200	& 614.600	& 6.3	& $\pm$ & 0.5 \\
614.600	& 615.050	& 6.3	& $\pm$ & 0.5 \\
615.050	& 615.450	& 6.3	& $\pm$ & 0.5 \\
615.450	& 615.850	& 6.3	& $\pm$ & 0.5 \\
615.850	& 616.250	& 6.4	& $\pm$ & 0.5 \\
616.250	& 616.650	& 6.5	& $\pm$ & 0.5 \\
616.650	& 617.050	& 6.6	& $\pm$ & 0.6 \\
617.050	& 617.450	& 6.5	& $\pm$ & 0.5 \\
617.450	& 617.850	& 6.6	& $\pm$ & 0.5 \\
617.850	& 618.250	& 6.7	& $\pm$ & 0.6 \\
618.250	& 618.650	& 6.7	& $\pm$ & 0.6 \\
618.650	& 619.050	& 6.8	& $\pm$ & 0.6 \\
619.050	& 619.450	& 6.9	& $\pm$ & 0.6 \\
619.450	& 619.850	& 7.0	& $\pm$ & 0.6 \\
619.850	& 620.250	& 7.1	& $\pm$ & 0.6 \\
620.250	& 620.650	& 7.0	& $\pm$ & 0.6 \\
620.650	& 621.050	& 7.2	& $\pm$ & 0.6 \\
621.050	& 621.450	& 7.0	& $\pm$ & 0.6 \\
621.450	& 621.800	& 6.9	& $\pm$ & 0.6 \\
621.800	& 622.200	& 6.9	& $\pm$ & 0.6 \\
622.200	& 622.600	& 6.9	& $\pm$ & 0.6 \\
622.600	& 623.000	& 6.9	& $\pm$ & 0.6 \\
623.000	& 623.400	& 6.4	& $\pm$ & 0.5 \\
623.400	& 623.800	& 6.7	& $\pm$ & 0.5 \\
623.800	& 624.150	& 6.6	& $\pm$ & 0.5 \\
624.150	& 624.550	& 6.7	& $\pm$ & 0.5 \\
624.550	& 624.950	& 6.6	& $\pm$ & 0.6 \\
624.950	& 625.350	& 6.5	& $\pm$ & 0.5 \\
625.350	& 625.750	& 6.5	& $\pm$ & 0.5 \\
625.750	& 626.100	& 6.4	& $\pm$ & 0.5 \\
626.100	& 626.500	& 6.3	& $\pm$ & 0.5 \\
626.500	& 627.000	& 6.3	& $\pm$ & 0.5 \\
627.000	& 627.350	& 6.4	& $\pm$ & 0.5 \\
627.350	& 627.750	& 6.4	& $\pm$ & 0.5 \\
627.750	& 628.150	& 6.2	& $\pm$ & 0.5 \\
628.150	& 628.550	& 6.2	& $\pm$ & 0.5 \\
628.550	& 628.900	& 6.1	& $\pm$ & 0.5 \\
628.900	& 629.300	& 6.1	& $\pm$ & 0.5 \\
629.300	& 629.700	& 6.1	& $\pm$ & 0.5 \\
629.700	& 630.050	& 6.1	& $\pm$ & 0.5 \\
630.050	& 630.450	& 6.1	& $\pm$ & 0.5 \\
630.450	& 630.850	& 6.3	& $\pm$ & 0.5 \\
630.850	& 631.200	& 6.3	& $\pm$ & 0.5 \\
631.200	& 631.600	& 6.2	& $\pm$ & 0.5 \\
631.600	& 631.950	& 6.3	& $\pm$ & 0.5 \\
631.950	& 632.350	& 6.2	& $\pm$ & 0.5 \\
632.350	& 632.750	& 6.1	& $\pm$ & 0.5 \\
632.750	& 633.100	& 6.0	& $\pm$ & 0.5 \\
633.100	& 633.500	& 6.0	& $\pm$ & 0.5 \\
633.500	& 633.850	& 6.0	& $\pm$ & 0.5 \\
633.850	& 634.250	& 6.1	& $\pm$ & 0.5 \\
634.250	& 634.650	& 6.1	& $\pm$ & 0.5 \\
634.650	& 635.000	& 6.1	& $\pm$ & 0.5 \\
635.000	& 636.450	& 6.0	& $\pm$ & 0.5 \\
636.450	& 636.800	& 6.0	& $\pm$ & 0.5 \\
636.800	& 637.200	& 6.0	& $\pm$ & 0.5 \\
637.200	& 637.550	& 6.0	& $\pm$ & 0.5 \\
637.550	& 637.950	& 6.0	& $\pm$ & 0.5 \\
637.950	& 638.300	& 6.0	& $\pm$ & 0.5 \\
638.300	& 638.650	& 6.1	& $\pm$ & 0.5 \\
638.650	& 639.050	& 6.2	& $\pm$ & 0.5 \\
639.050	& 639.400	& 6.2	& $\pm$ & 0.5 \\
639.400	& 639.800	& 6.1	& $\pm$ & 0.5 \\
639.800	& 640.150	& 6.1	& $\pm$ & 0.5 \\
640.150	& 640.550	& 6.2	& $\pm$ & 0.5 \\
640.550	& 640.900	& 6.2	& $\pm$ & 0.5 \\
640.900	& 641.250	& 6.2	& $\pm$ & 0.5 \\
641.250	& 641.650	& 6.1	& $\pm$ & 0.5 \\
641.650	& 642.000	& 6.1	& $\pm$ & 0.5 \\
642.000	& 642.400	& 6.1	& $\pm$ & 0.5 \\
642.400	& 642.750	& 6.1	& $\pm$ & 0.5 \\
642.750	& 643.100	& 6.1	& $\pm$ & 0.5 \\
643.100	& 643.500	& 6.1	& $\pm$ & 0.5 \\
643.500	& 643.850	& 6.2	& $\pm$ & 0.5 \\
643.850	& 644.200	& 6.3	& $\pm$ & 0.5 \\
644.200	& 644.600	& 6.2	& $\pm$ & 0.5 \\
644.600	& 644.950	& 6.1	& $\pm$ & 0.5 \\
644.950	& 645.300	& 6.1	& $\pm$ & 0.5 \\
645.300	& 647.250	& 6.1	& $\pm$ & 0.5 \\
647.250	& 647.650	& 6.1	& $\pm$ & 0.5 \\
647.650	& 648.000	& 6.1	& $\pm$ & 0.5 \\
648.000	& 649.250	& 6.1	& $\pm$ & 0.5 \\
649.250	& 649.650	& 6.1	& $\pm$ & 0.5 \\
649.650	& 650.050	& 6.1	& $\pm$ & 0.5 \\
650.050	& 650.400	& 6.2	& $\pm$ & 0.5 \\
650.400	& 650.750	& 6.1	& $\pm$ & 0.5 \\
650.750	& 651.100	& 6.1	& $\pm$ & 0.5 \\
651.100	& 651.450	& 6.2	& $\pm$ & 0.5 \\
651.450	& 651.800	& 6.2	& $\pm$ & 0.5 \\
651.800	& 652.200	& 6.2	& $\pm$ & 0.5 \\
652.200	& 652.700	& 6.3	& $\pm$ & 0.5 \\
652.700	& 653.050	& 6.3	& $\pm$ & 0.5 \\
653.050	& 653.400	& 6.2	& $\pm$ & 0.5 \\
653.400	& 653.750	& 6.3	& $\pm$ & 0.5 \\
653.750	& 654.100	& 6.2	& $\pm$ & 0.5 \\
654.100	& 654.450	& 6.6	& $\pm$ & 0.5 \\
654.450	& 654.800	& 6.6	& $\pm$ & 0.5 \\
654.800	& 655.200	& 6.3	& $\pm$ & 0.5 \\
655.200	& 655.550	& 6.3	& $\pm$ & 0.5 \\
655.550	& 655.900	& 6.3	& $\pm$ & 0.5 \\
655.900	& 656.250	& 6.3	& $\pm$ & 0.5 \\
656.250	& 656.600	& 6.2	& $\pm$ & 0.5 \\
656.600	& 656.950	& 6.3	& $\pm$ & 0.5 \\
656.950	& 657.300	& 6.4	& $\pm$ & 0.5 \\
657.300	& 657.650	& 6.2	& $\pm$ & 0.5 \\
657.650	& 658.000	& 6.2	& $\pm$ & 0.5 \\
658.000	& 660.350	& 6.2	& $\pm$ & 0.5 \\
660.350	& 660.700	& 6.2	& $\pm$ & 0.5 \\
660.700	& 661.050	& 6.2	& $\pm$ & 0.5 \\
661.050	& 661.400	& 6.3	& $\pm$ & 0.5 \\
661.400	& 661.750	& 6.2	& $\pm$ & 0.5 \\
661.750	& 662.100	& 6.3	& $\pm$ & 0.5 \\
662.100	& 662.450	& 6.2	& $\pm$ & 0.5 \\
662.450	& 662.800	& 6.3	& $\pm$ & 0.5 \\
662.800	& 663.100	& 6.3	& $\pm$ & 0.5 \\
663.100	& 663.450	& 6.4	& $\pm$ & 0.5 \\
663.450	& 663.800	& 6.3	& $\pm$ & 0.5 \\
663.800	& 664.350	& 6.4	& $\pm$ & 0.5 \\
664.350	& 664.700	& 6.4	& $\pm$ & 0.5 \\
664.700	& 665.050	& 6.3	& $\pm$ & 0.5 \\
665.050	& 665.400	& 6.3	& $\pm$ & 0.5 \\
665.400	& 665.750	& 6.4	& $\pm$ & 0.5 \\
665.750	& 666.100	& 6.3	& $\pm$ & 0.5 \\
666.100	& 666.500	& 6.3	& $\pm$ & 0.5 \\
666.500	& 666.850	& 6.4	& $\pm$ & 0.5 \\
666.850	& 667.200	& 6.4	& $\pm$ & 0.5 \\
667.200	& 667.550	& 6.4	& $\pm$ & 0.5 \\
667.550	& 667.900	& 6.4	& $\pm$ & 0.5 \\
667.900	& 668.200	& 6.5	& $\pm$ & 0.5 \\
668.200	& 668.550	& 6.7	& $\pm$ & 0.6 \\
668.550	& 668.900	& 6.9	& $\pm$ & 0.6 \\
668.900	& 669.250	& 6.5	& $\pm$ & 0.5 \\
669.250	& 669.600	& 6.4	& $\pm$ & 0.5 \\
669.600	& 669.900	& 6.4	& $\pm$ & 0.5 \\
669.900	& 670.250	& 6.4	& $\pm$ & 0.5 \\
670.250	& 670.600	& 6.4	& $\pm$ & 0.5 \\
670.600	& 670.950	& 6.4	& $\pm$ & 0.5 \\
670.950	& 671.250	& 6.5	& $\pm$ & 0.5 \\
671.250	& 671.600	& 6.4	& $\pm$ & 0.5 \\
671.600	& 671.950	& 6.4	& $\pm$ & 0.5 \\
671.950	& 672.300	& 6.6	& $\pm$ & 0.6 \\
672.300	& 672.600	& 6.6	& $\pm$ & 0.6 \\
672.600	& 672.950	& 6.5	& $\pm$ & 0.5 \\
672.950	& 673.300	& 6.4	& $\pm$ & 0.5 \\
673.300	& 673.650	& 6.4	& $\pm$ & 0.5 \\
673.650	& 673.950	& 6.4	& $\pm$ & 0.5 \\
673.950	& 674.300	& 6.4	& $\pm$ & 0.5 \\
674.300	& 674.650	& 6.4	& $\pm$ & 0.5 \\
674.650	& 674.950	& 6.4	& $\pm$ & 0.5 \\
674.950	& 675.300	& 6.5	& $\pm$ & 0.5 \\
675.300	& 675.650	& 6.5	& $\pm$ & 0.5 \\
675.650	& 675.950	& 6.6	& $\pm$ & 0.6 \\
675.950	& 676.300	& 6.5	& $\pm$ & 0.5 \\
676.300	& 676.650	& 6.6	& $\pm$ & 0.5 \\
676.650	& 676.950	& 6.8	& $\pm$ & 0.6 \\
676.950	& 677.300	& 6.6	& $\pm$ & 0.5 \\
677.300	& 677.600	& 6.5	& $\pm$ & 0.5 \\
677.600	& 677.950	& 6.5	& $\pm$ & 0.5 \\
677.950	& 678.300	& 6.5	& $\pm$ & 0.5 \\
678.300	& 678.600	& 6.5	& $\pm$ & 0.5 \\
678.600	& 678.950	& 6.6	& $\pm$ & 0.5 \\
678.950	& 679.250	& 6.7	& $\pm$ & 0.5 \\
679.250	& 679.600	& 6.6	& $\pm$ & 0.5 \\
679.600	& 679.950	& 6.6	& $\pm$ & 0.5 \\
679.950	& 680.250	& 6.8	& $\pm$ & 0.6 \\
680.250	& 680.600	& 6.6	& $\pm$ & 0.5 \\
680.600	& 680.900	& 6.7	& $\pm$ & 0.5 \\
680.900	& 681.250	& 6.6	& $\pm$ & 0.5 \\
681.250	& 681.550	& 6.8	& $\pm$ & 0.6 \\
681.550	& 681.900	& 6.7	& $\pm$ & 0.6 \\
681.900	& 682.200	& 6.6	& $\pm$ & 0.5 \\
682.200	& 682.550	& 6.6	& $\pm$ & 0.5 \\
682.550	& 682.900	& 6.8	& $\pm$ & 0.6 \\
682.900	& 683.200	& 6.8	& $\pm$ & 0.6 \\
683.200	& 683.550	& 6.6	& $\pm$ & 0.5 \\
683.550	& 683.850	& 6.6	& $\pm$ & 0.5 \\
683.850	& 684.200	& 6.6	& $\pm$ & 0.5 \\
684.200	& 684.500	& 6.7	& $\pm$ & 0.5 \\
684.500	& 684.850	& 6.7	& $\pm$ & 0.6 \\
684.850	& 685.150	& 6.9	& $\pm$ & 0.6 \\
685.150	& 685.500	& 6.8	& $\pm$ & 0.6 \\
685.500	& 685.850	& 6.8	& $\pm$ & 0.6 \\
685.850	& 690.650	& 6.9	& $\pm$ & 0.6 \\
690.650	& 691.000	& 7.0	& $\pm$ & 0.6 \\
691.000	& 691.300	& 7.2	& $\pm$ & 0.6 \\
691.300	& 691.600	& 7.3	& $\pm$ & 0.6 \\
691.600	& 692.650	& 7.3	& $\pm$ & 0.6 \\
692.650	& 695.250	& 7.5	& $\pm$ & 0.6 \\
695.250	& 695.750	& 8.0	& $\pm$ & 0.7 \\
695.750	& 696.200	& 9.1	& $\pm$ & 0.7 \\
696.200	& 696.500	& 10.2	& $\pm$ & 0.8 \\
696.500	& 696.800	& 8.7	& $\pm$ & 0.7 \\
696.800	& 697.150	& 9.3	& $\pm$ & 0.8 \\
697.150	& 697.450	& 8.6	& $\pm$ & 0.7 \\
697.450	& 697.750	& 8.9	& $\pm$ & 0.7 \\
697.750	& 698.050	& 12.6	& $\pm$ & 1.0 \\
698.050	& 698.350	& 12.8	& $\pm$ & 1.0 \\
698.350	& 698.700	& 10.5	& $\pm$ & 0.9 \\
698.700	& 699.000	& 9.5	& $\pm$ & 0.8 \\
699.000	& 699.300	& 8.3	& $\pm$ & 0.7 \\
699.300	& 699.600	& 7.9	& $\pm$ & 0.7 \\
699.600	& 699.950	& 7.8	& $\pm$ & 0.6 \\
699.950	& 700.250	& 7.6	& $\pm$ & 0.6 \\
700.250	& 700.550	& 7.5	& $\pm$ & 0.6 \\
700.550	& 700.850	& 7.3	& $\pm$ & 0.6 \\
700.850	& 701.150	& 7.2	& $\pm$ & 0.6 \\
701.150	& 701.500	& 7.3	& $\pm$ & 0.6 \\
701.500	& 701.800	& 7.3	& $\pm$ & 0.6 \\
701.800	& 702.100	& 7.1	& $\pm$ & 0.6 \\
702.100	& 702.400	& 7.0	& $\pm$ & 0.6 \\
702.400	& 702.700	& 7.0	& $\pm$ & 0.6 \\
702.700	& 703.000	& 7.0	& $\pm$ & 0.6 \\
703.000	& 704.550	& 7.2	& $\pm$ & 0.6 \\
704.550	& 704.900	& 7.1	& $\pm$ & 0.6 \\
704.900	& 705.200	& 7.2	& $\pm$ & 0.6 \\
705.200	& 705.500	& 7.4	& $\pm$ & 0.6 \\
705.500	& 705.800	& 7.1	& $\pm$ & 0.6 \\
705.800	& 706.100	& 7.0	& $\pm$ & 0.6 \\
706.100	& 706.400	& 7.0	& $\pm$ & 0.6 \\
706.400	& 706.700	& 6.9	& $\pm$ & 0.6 \\
706.700	& 707.000	& 6.9	& $\pm$ & 0.6 \\
707.000	& 707.300	& 6.9	& $\pm$ & 0.6 \\
707.300	& 707.600	& 6.8	& $\pm$ & 0.6 \\
707.600	& 707.950	& 6.8	& $\pm$ & 0.6 \\
707.950	& 708.250	& 6.9	& $\pm$ & 0.6 \\
708.250	& 708.550	& 6.9	& $\pm$ & 0.6 \\
708.550	& 708.850	& 7.0	& $\pm$ & 0.6 \\
708.850	& 709.150	& 6.9	& $\pm$ & 0.6 \\
709.150	& 709.450	& 6.9	& $\pm$ & 0.6 \\
709.450	& 709.750	& 6.9	& $\pm$ & 0.6 \\
709.750	& 710.050	& 6.9	& $\pm$ & 0.6 \\
710.050	& 710.350	& 7.0	& $\pm$ & 0.6 \\
710.350	& 710.650	& 7.1	& $\pm$ & 0.6 \\
710.650	& 710.950	& 7.2	& $\pm$ & 0.6 \\
710.950	& 711.250	& 7.2	& $\pm$ & 0.6 \\
711.250	& 711.550	& 7.1	& $\pm$ & 0.6 \\
711.550	& 711.850	& 7.1	& $\pm$ & 0.6 \\
711.850	& 712.150	& 7.1	& $\pm$ & 0.6 \\
712.150	& 712.450	& 7.0	& $\pm$ & 0.6 \\
712.450	& 712.750	& 7.0	& $\pm$ & 0.6 \\
712.750	& 713.050	& 7.0	& $\pm$ & 0.6 \\
713.050	& 713.350	& 7.0	& $\pm$ & 0.6 \\
713.350	& 713.650	& 7.1	& $\pm$ & 0.6 \\
713.650	& 713.950	& 7.0	& $\pm$ & 0.6 \\
713.950	& 714.250	& 7.0	& $\pm$ & 0.6 \\
714.250	& 714.550	& 7.0	& $\pm$ & 0.6 \\
714.550	& 714.850	& 7.0	& $\pm$ & 0.6 \\
714.850	& 715.150	& 7.0	& $\pm$ & 0.6 \\
715.150	& 715.450	& 7.0	& $\pm$ & 0.6 \\
715.450	& 715.750	& 6.9	& $\pm$ & 0.6 \\
715.750	& 716.000	& 7.0	& $\pm$ & 0.6 \\
716.000	& 716.300	& 7.0	& $\pm$ & 0.6 \\
716.300	& 716.600	& 7.1	& $\pm$ & 0.6 \\
716.600	& 716.900	& 7.0	& $\pm$ & 0.6 \\
716.900	& 717.200	& 7.1	& $\pm$ & 0.6 \\
717.200	& 717.500	& 7.0	& $\pm$ & 0.6 \\
717.500	& 717.800	& 7.0	& $\pm$ & 0.6 \\
717.800	& 718.100	& 6.9	& $\pm$ & 0.6 \\
718.100	& 718.400	& 6.9	& $\pm$ & 0.6 \\
718.400	& 718.700	& 7.0	& $\pm$ & 0.6 \\
718.700	& 718.950	& 6.9	& $\pm$ & 0.6 \\
718.950	& 719.250	& 7.0	& $\pm$ & 0.6 \\
719.250	& 719.550	& 6.9	& $\pm$ & 0.6 \\
719.550	& 719.850	& 6.9	& $\pm$ & 0.6 \\
719.850	& 720.150	& 6.9	& $\pm$ & 0.6 \\
720.150	& 720.450	& 6.9	& $\pm$ & 0.6 \\
720.450	& 720.750	& 6.9	& $\pm$ & 0.6 \\
720.750	& 721.050	& 6.9	& $\pm$ & 0.6 \\
721.050	& 721.300	& 6.9	& $\pm$ & 0.6 \\
721.300	& 721.600	& 6.9	& $\pm$ & 0.6 \\
721.600	& 721.900	& 6.9	& $\pm$ & 0.6 \\
721.900	& 722.200	& 7.2	& $\pm$ & 0.6 \\
722.200	& 722.500	& 7.1	& $\pm$ & 0.6 \\
722.500	& 722.800	& 7.1	& $\pm$ & 0.6 \\
722.800	& 723.050	& 6.9	& $\pm$ & 0.6 \\
723.050	& 723.350	& 7.1	& $\pm$ & 0.6 \\
723.350	& 723.650	& 6.9	& $\pm$ & 0.6 \\
723.650	& 723.950	& 7.0	& $\pm$ & 0.6 \\
723.950	& 724.250	& 7.0	& $\pm$ & 0.6 \\
724.250	& 724.500	& 7.2	& $\pm$ & 0.6 \\
724.500	& 724.800	& 7.1	& $\pm$ & 0.6 \\
724.800	& 725.100	& 7.0	& $\pm$ & 0.6 \\
725.100	& 725.400	& 6.9	& $\pm$ & 0.6 \\
725.400	& 725.700	& 6.9	& $\pm$ & 0.6 \\
725.700	& 725.950	& 6.9	& $\pm$ & 0.6 \\
725.950	& 726.250	& 7.0	& $\pm$ & 0.6 \\
726.250	& 726.550	& 6.9	& $\pm$ & 0.6 \\
726.550	& 726.850	& 7.0	& $\pm$ & 0.6 \\
726.850	& 727.100	& 6.9	& $\pm$ & 0.6 \\
727.100	& 727.400	& 7.0	& $\pm$ & 0.6 \\
727.400	& 727.700	& 7.0	& $\pm$ & 0.6 \\
727.700	& 728.000	& 6.9	& $\pm$ & 0.6 \\
728.000	& 728.250	& 6.9	& $\pm$ & 0.6 \\
728.250	& 728.550	& 7.1	& $\pm$ & 0.6 \\
728.550	& 728.850	& 6.9	& $\pm$ & 0.6 \\
728.850	& 729.100	& 7.0	& $\pm$ & 0.6 \\
729.100	& 730.250	& 7.0	& $\pm$ & 0.6 \\
730.250	& 730.550	& 7.0	& $\pm$ & 0.6 \\
730.550	& 730.850	& 7.0	& $\pm$ & 0.6 \\
730.850	& 731.100	& 7.0	& $\pm$ & 0.6 \\
731.100	& 731.400	& 7.0	& $\pm$ & 0.6 \\
731.400	& 731.700	& 7.1	& $\pm$ & 0.6 \\
731.700	& 731.950	& 7.1	& $\pm$ & 0.6 \\
731.950	& 732.250	& 7.0	& $\pm$ & 0.6 \\
732.250	& 732.550	& 7.0	& $\pm$ & 0.6 \\
732.550	& 732.800	& 7.1	& $\pm$ & 0.6 \\
732.800	& 733.100	& 7.1	& $\pm$ & 0.6 \\
733.100	& 733.400	& 7.1	& $\pm$ & 0.6 \\
733.400	& 733.650	& 7.2	& $\pm$ & 0.6 \\
733.650	& 733.950	& 7.1	& $\pm$ & 0.6 \\
733.950	& 734.250	& 7.1	& $\pm$ & 0.6 \\
734.250	& 734.500	& 7.1	& $\pm$ & 0.6 \\
734.500	& 734.800	& 7.1	& $\pm$ & 0.6 \\
734.800	& 735.050	& 7.0	& $\pm$ & 0.6 \\
735.050	& 735.350	& 7.0	& $\pm$ & 0.6 \\
735.350	& 735.650	& 7.0	& $\pm$ & 0.6 \\
735.650	& 735.900	& 7.1	& $\pm$ & 0.6 \\
735.900	& 736.200	& 7.1	& $\pm$ & 0.6 \\
736.200	& 736.500	& 7.1	& $\pm$ & 0.6 \\
736.500	& 736.750	& 7.2	& $\pm$ & 0.6 \\
736.750	& 737.050	& 7.4	& $\pm$ & 0.6 \\
737.050	& 737.300	& 7.3	& $\pm$ & 0.6 \\
737.300	& 737.600	& 7.2	& $\pm$ & 0.6 \\
737.600	& 737.850	& 7.3	& $\pm$ & 0.6 \\
737.850	& 738.150	& 7.1	& $\pm$ & 0.6 \\
738.150	& 738.450	& 7.1	& $\pm$ & 0.6 \\
738.450	& 738.700	& 7.1	& $\pm$ & 0.6 \\
738.700	& 739.000	& 7.1	& $\pm$ & 0.6 \\
739.000	& 739.250	& 7.1	& $\pm$ & 0.6 \\
739.250	& 739.550	& 7.1	& $\pm$ & 0.6 \\
739.550	& 739.800	& 7.1	& $\pm$ & 0.6 \\
739.800	& 740.100	& 7.1	& $\pm$ & 0.6 \\
740.100	& 740.400	& 7.1	& $\pm$ & 0.6 \\
740.400	& 740.650	& 7.1	& $\pm$ & 0.6 \\
740.650	& 740.950	& 7.2	& $\pm$ & 0.6 \\
740.950	& 741.200	& 7.1	& $\pm$ & 0.6 \\
741.200	& 741.500	& 7.2	& $\pm$ & 0.6 \\
741.500	& 741.750	& 7.2	& $\pm$ & 0.6 \\
741.750	& 742.050	& 7.1	& $\pm$ & 0.6 \\
742.050	& 742.300	& 7.1	& $\pm$ & 0.6 \\
742.300	& 742.600	& 7.1	& $\pm$ & 0.6 \\
742.600	& 742.850	& 7.1	& $\pm$ & 0.6 \\
742.850	& 743.150	& 7.1	& $\pm$ & 0.6 \\
743.150	& 743.400	& 7.1	& $\pm$ & 0.6 \\
743.400	& 743.700	& 7.1	& $\pm$ & 0.6 \\
743.700	& 743.950	& 7.1	& $\pm$ & 0.6 \\
743.950	& 744.250	& 7.1	& $\pm$ & 0.6 \\
744.250	& 744.500	& 7.1	& $\pm$ & 0.6 \\
744.500	& 744.800	& 7.1	& $\pm$ & 0.6 \\
744.800	& 745.050	& 7.1	& $\pm$ & 0.6 \\
745.050	& 745.350	& 7.3	& $\pm$ & 0.6 \\
745.350	& 745.600	& 7.1	& $\pm$ & 0.6 \\
745.600	& 745.900	& 7.1	& $\pm$ & 0.6 \\
745.900	& 746.150	& 7.1	& $\pm$ & 0.6 \\
746.150	& 746.450	& 7.1	& $\pm$ & 0.6 \\
746.450	& 746.700	& 7.3	& $\pm$ & 0.6 \\
746.700	& 746.950	& 7.2	& $\pm$ & 0.6 \\
746.950	& 747.250	& 7.2	& $\pm$ & 0.6 \\
747.250	& 747.500	& 7.1	& $\pm$ & 0.6 \\
747.500	& 747.800	& 7.1	& $\pm$ & 0.6 \\
747.800	& 748.050	& 7.1	& $\pm$ & 0.6 \\
748.050	& 748.350	& 7.2	& $\pm$ & 0.6 \\
748.350	& 748.600	& 7.1	& $\pm$ & 0.6 \\
748.600	& 748.900	& 7.1	& $\pm$ & 0.6 \\
748.900	& 749.150	& 7.2	& $\pm$ & 0.6 \\
749.150	& 749.400	& 7.2	& $\pm$ & 0.6 \\
749.400	& 749.700	& 7.1	& $\pm$ & 0.6 \\
749.700	& 749.950	& 7.3	& $\pm$ & 0.6 \\
749.950	& 750.250	& 7.2	& $\pm$ & 0.6 \\
750.250	& 750.500	& 7.2	& $\pm$ & 0.6 \\
750.500	& 750.750	& 7.2	& $\pm$ & 0.6 \\
750.750	& 751.050	& 7.2	& $\pm$ & 0.6 \\
751.050	& 751.300	& 7.2	& $\pm$ & 0.6 \\
751.300	& 751.600	& 7.2	& $\pm$ & 0.6 \\
751.600	& 751.850	& 7.2	& $\pm$ & 0.6 \\
751.850	& 752.100	& 7.2	& $\pm$ & 0.6 \\
752.100	& 752.400	& 7.3	& $\pm$ & 0.6 \\
752.400	& 752.650	& 7.3	& $\pm$ & 0.6 \\
752.650	& 752.900	& 7.2	& $\pm$ & 0.6 \\
752.900	& 753.200	& 7.3	& $\pm$ & 0.6 \\
753.200	& 753.450	& 7.2	& $\pm$ & 0.6 \\
753.450	& 753.700	& 7.3	& $\pm$ & 0.6 \\
753.700	& 754.000	& 7.4	& $\pm$ & 0.6 \\
754.000	& 754.250	& 7.4	& $\pm$ & 0.6 \\
754.250	& 754.550	& 7.3	& $\pm$ & 0.6 \\
754.550	& 754.800	& 7.3	& $\pm$ & 0.6 \\
754.800	& 755.050	& 7.3	& $\pm$ & 0.6 \\
755.050	& 755.350	& 7.3	& $\pm$ & 0.6 \\
755.350	& 755.650	& 7.2	& $\pm$ & 0.6 \\
755.650	& 755.900	& 7.2	& $\pm$ & 0.6 \\
755.900	& 756.150	& 7.3	& $\pm$ & 0.6 \\
756.150	& 756.450	& 7.2	& $\pm$ & 0.6 \\
756.450	& 756.700	& 7.2	& $\pm$ & 0.6 \\
756.700	& 756.950	& 7.2	& $\pm$ & 0.6 \\
756.950	& 757.250	& 7.2	& $\pm$ & 0.6 \\
757.250	& 757.500	& 7.2	& $\pm$ & 0.6 \\
757.500	& 757.850	& 7.2	& $\pm$ & 0.6 \\
757.850	& 758.200	& 7.2	& $\pm$ & 0.6 \\
758.200	& 758.450	& 7.3	& $\pm$ & 0.6 \\
758.450	& 758.700	& 7.2	& $\pm$ & 0.6 \\
758.700	& 758.950	& 7.2	& $\pm$ & 0.6 \\
758.950	& 759.250	& 7.2	& $\pm$ & 0.6 \\
759.250	& 759.500	& 7.2	& $\pm$ & 0.6 \\
759.500	& 759.750	& 7.3	& $\pm$ & 0.6 \\
759.750	& 760.050	& 7.3	& $\pm$ & 0.6 \\
760.050	& 760.300	& 7.3	& $\pm$ & 0.6 \\
760.300	& 760.550	& 7.3	& $\pm$ & 0.6 \\
760.550	& 760.800	& 7.3	& $\pm$ & 0.6 \\
760.800	& 761.100	& 7.3	& $\pm$ & 0.6 \\
761.100	& 761.350	& 7.3	& $\pm$ & 0.6 \\
761.350	& 761.600	& 7.3	& $\pm$ & 0.6 \\
761.600	& 761.850	& 7.4	& $\pm$ & 0.6 \\
761.850	& 762.150	& 7.9	& $\pm$ & 0.6 \\
762.150	& 762.400	& 7.7	& $\pm$ & 0.6 \\
762.400	& 762.650	& 7.4	& $\pm$ & 0.6 \\
762.650	& 762.900	& 7.5	& $\pm$ & 0.6 \\
762.900	& 763.150	& 7.5	& $\pm$ & 0.6 \\
763.150	& 763.450	& 7.5	& $\pm$ & 0.6 \\
763.450	& 763.700	& 7.5	& $\pm$ & 0.6 \\
763.700	& 763.950	& 7.7	& $\pm$ & 0.6 \\
763.950	& 764.200	& 7.9	& $\pm$ & 0.6 \\
764.200	& 764.450	& 7.6	& $\pm$ & 0.6 \\
764.450	& 764.750	& 7.6	& $\pm$ & 0.6 \\
764.750	& 765.000	& 7.6	& $\pm$ & 0.6 \\
765.000	& 765.250	& 7.5	& $\pm$ & 0.6 \\
765.250	& 765.500	& 7.5	& $\pm$ & 0.6 \\
765.500	& 765.750	& 7.4	& $\pm$ & 0.6 \\
765.750	& 766.050	& 7.4	& $\pm$ & 0.6 \\
766.050	& 766.300	& 7.5	& $\pm$ & 0.6 \\
766.300	& 766.550	& 7.4	& $\pm$ & 0.6 \\
766.550	& 766.800	& 7.4	& $\pm$ & 0.6 \\
766.800	& 767.050	& 7.5	& $\pm$ & 0.6 \\
767.050	& 767.350	& 7.4	& $\pm$ & 0.6 \\
767.350	& 767.650	& 7.3	& $\pm$ & 0.6 \\
767.650	& 767.900	& 7.3	& $\pm$ & 0.6 \\
767.900	& 768.150	& 7.3	& $\pm$ & 0.6 \\
768.150	& 768.400	& 7.3	& $\pm$ & 0.6 \\
768.400	& 768.650	& 7.3	& $\pm$ & 0.6 \\
768.650	& 768.900	& 7.3	& $\pm$ & 0.6 \\
768.900	& 769.200	& 7.3	& $\pm$ & 0.6 \\
769.200	& 769.450	& 7.3	& $\pm$ & 0.6 \\
769.450	& 769.700	& 7.3	& $\pm$ & 0.6 \\
769.700	& 769.950	& 7.3	& $\pm$ & 0.6 \\
769.950	& 770.200	& 7.3	& $\pm$ & 0.6 \\
770.200	& 770.450	& 7.4	& $\pm$ & 0.6 \\
770.450	& 770.700	& 7.3	& $\pm$ & 0.6 \\
770.700	& 770.950	& 7.4	& $\pm$ & 0.6 \\
770.950	& 771.250	& 7.3	& $\pm$ & 0.6 \\
771.250	& 771.500	& 7.5	& $\pm$ & 0.6 \\
771.500	& 771.750	& 7.3	& $\pm$ & 0.6 \\
771.750	& 772.000	& 7.3	& $\pm$ & 0.6 \\
772.000	& 772.250	& 7.3	& $\pm$ & 0.6 \\
772.250	& 772.500	& 7.3	& $\pm$ & 0.6 \\
772.500	& 772.750	& 7.6	& $\pm$ & 0.6 \\
772.750	& 773.000	& 7.3	& $\pm$ & 0.6 \\
773.000	& 773.250	& 7.3	& $\pm$ & 0.6 \\
773.250	& 773.500	& 7.3	& $\pm$ & 0.6 \\
773.500	& 773.750	& 7.3	& $\pm$ & 0.6 \\
773.750	& 774.050	& 7.3	& $\pm$ & 0.6 \\
774.050	& 774.300	& 7.3	& $\pm$ & 0.6 \\
774.300	& 774.550	& 7.3	& $\pm$ & 0.6 \\
774.550	& 774.800	& 7.3	& $\pm$ & 0.6 \\
774.800	& 775.050	& 7.3	& $\pm$ & 0.6 \\
775.050	& 775.300	& 7.3	& $\pm$ & 0.6 \\
775.300	& 775.550	& 7.3	& $\pm$ & 0.6 \\
775.550	& 775.800	& 7.4	& $\pm$ & 0.6 \\
775.800	& 776.050	& 7.3	& $\pm$ & 0.6 \\
776.050	& 776.300	& 7.3	& $\pm$ & 0.6 \\
776.300	& 776.550	& 7.3	& $\pm$ & 0.6 \\
776.550	& 776.800	& 7.3	& $\pm$ & 0.6 \\
776.800	& 777.050	& 7.3	& $\pm$ & 0.6 \\
777.050	& 777.300	& 7.3	& $\pm$ & 0.6 \\
777.300	& 777.550	& 7.3	& $\pm$ & 0.6 \\
777.550	& 777.800	& 7.4	& $\pm$ & 0.6 \\
777.800	& 778.050	& 7.4	& $\pm$ & 0.6 \\
778.050	& 778.300	& 7.4	& $\pm$ & 0.6 \\
778.300	& 778.550	& 7.4	& $\pm$ & 0.6 \\
778.550	& 778.800	& 7.4	& $\pm$ & 0.6 \\
778.800	& 779.050	& 7.4	& $\pm$ & 0.6 \\
779.050	& 779.300	& 7.4	& $\pm$ & 0.6 \\
779.300	& 779.550	& 7.5	& $\pm$ & 0.6 \\
779.550	& 779.800	& 7.4	& $\pm$ & 0.6 \\
779.800	& 780.050	& 7.4	& $\pm$ & 0.6 \\
780.050	& 780.300	& 7.4	& $\pm$ & 0.6 \\
780.300	& 780.550	& 7.4	& $\pm$ & 0.6 \\
780.550	& 780.800	& 7.4	& $\pm$ & 0.6 \\
780.800	& 781.050	& 7.4	& $\pm$ & 0.6 \\
781.050	& 781.300	& 7.7	& $\pm$ & 0.6 \\
781.300	& 781.550	& 7.4	& $\pm$ & 0.6 \\
781.550	& 781.800	& 7.4	& $\pm$ & 0.6 \\
781.800	& 782.050	& 7.7	& $\pm$ & 0.6 \\
782.050	& 782.300	& 7.4	& $\pm$ & 0.6 \\
782.300	& 782.550	& 7.4	& $\pm$ & 0.6 \\
782.550	& 782.800	& 7.4	& $\pm$ & 0.6 \\
782.800	& 783.050	& 7.4	& $\pm$ & 0.6 \\
783.050	& 783.300	& 7.4	& $\pm$ & 0.6 \\
783.300	& 783.550	& 7.4	& $\pm$ & 0.6 \\
783.550	& 783.800	& 7.4	& $\pm$ & 0.6 \\
783.800	& 784.050	& 7.6	& $\pm$ & 0.6 \\
784.050	& 784.300	& 7.4	& $\pm$ & 0.6 \\
784.300	& 784.550	& 7.4	& $\pm$ & 0.6 \\
784.550	& 784.800	& 7.4	& $\pm$ & 0.6 \\
784.800	& 785.050	& 7.4	& $\pm$ & 0.6 \\
785.050	& 785.300	& 7.5	& $\pm$ & 0.6 \\
785.300	& 785.550	& 7.5	& $\pm$ & 0.6 \\
785.550	& 785.750	& 7.4	& $\pm$ & 0.6 \\
785.750	& 786.050	& 7.5	& $\pm$ & 0.6 \\
786.050	& 786.300	& 7.4	& $\pm$ & 0.6 \\
786.300	& 786.550	& 7.4	& $\pm$ & 0.6 \\
786.550	& 786.800	& 7.4	& $\pm$ & 0.6 \\
786.800	& 787.050	& 7.4	& $\pm$ & 0.6 \\
787.050	& 787.300	& 7.5	& $\pm$ & 0.6 \\
787.300	& 787.550	& 7.4	& $\pm$ & 0.6 \\
787.550	& 787.800	& 7.4	& $\pm$ & 0.6 \\
787.800	& 788.050	& 7.5	& $\pm$ & 0.6 \\
788.050	& 788.300	& 7.6	& $\pm$ & 0.6 \\
788.300	& 788.500	& 7.4	& $\pm$ & 0.6 \\
788.500	& 788.750	& 7.5	& $\pm$ & 0.6 \\
788.750	& 789.000	& 7.5	& $\pm$ & 0.6 \\
789.000	& 789.250	& 7.5	& $\pm$ & 0.6 \\
789.250	& 789.500	& 7.5	& $\pm$ & 0.6 \\
789.500	& 789.750	& 7.7	& $\pm$ & 0.6 \\
789.750	& 790.000	& 7.5	& $\pm$ & 0.6 \\
790.000	& 790.250	& 7.5	& $\pm$ & 0.6 \\
790.250	& 790.450	& 7.5	& $\pm$ & 0.6 \\
790.450	& 790.700	& 7.4	& $\pm$ & 0.6 \\
790.700	& 790.950	& 7.4	& $\pm$ & 0.6 \\
790.950	& 791.200	& 7.5	& $\pm$ & 0.6 \\
791.200	& 791.450	& 7.6	& $\pm$ & 0.6 \\
791.450	& 791.700	& 7.5	& $\pm$ & 0.6 \\
791.700	& 791.950	& 7.7	& $\pm$ & 0.6 \\
791.950	& 792.150	& 7.5	& $\pm$ & 0.6 \\
792.150	& 792.400	& 7.5	& $\pm$ & 0.6 \\
792.400	& 792.650	& 7.5	& $\pm$ & 0.6 \\
792.650	& 792.900	& 7.5	& $\pm$ & 0.6 \\
792.900	& 793.250	& 7.6	& $\pm$ & 0.6 \\
793.250	& 793.500	& 7.5	& $\pm$ & 0.6 \\
793.500	& 793.700	& 7.5	& $\pm$ & 0.6 \\
793.700	& 793.950	& 7.5	& $\pm$ & 0.6 \\
793.950	& 794.200	& 7.5	& $\pm$ & 0.6 \\
794.200	& 794.450	& 7.5	& $\pm$ & 0.6 \\
794.450	& 794.700	& 7.5	& $\pm$ & 0.6 \\
794.700	& 794.950	& 7.7	& $\pm$ & 0.6 \\
794.950	& 795.150	& 7.5	& $\pm$ & 0.6 \\
795.150	& 795.400	& 7.6	& $\pm$ & 0.6 \\
795.400	& 795.650	& 7.6	& $\pm$ & 0.6 \\
795.650	& 795.900	& 7.6	& $\pm$ & 0.6 \\
795.900	& 796.150	& 7.5	& $\pm$ & 0.6 \\
796.150	& 796.350	& 7.7	& $\pm$ & 0.6 \\
796.350	& 798.000	& 7.6	& $\pm$ & 0.6 \\
798.000	& 798.250	& 7.6	& $\pm$ & 0.6 \\
798.250	& 798.500	& 7.7	& $\pm$ & 0.6 \\
798.500	& 798.700	& 7.6	& $\pm$ & 0.6 \\
798.700	& 798.950	& 7.6	& $\pm$ & 0.6 \\
798.950	& 799.200	& 7.6	& $\pm$ & 0.6 \\
799.200	& 800.350	& 7.6	& $\pm$ & 0.6 \\
800.350	& 801.750	& 7.7	& $\pm$ & 0.6 \\
801.750	& 802.000	& 7.8	& $\pm$ & 0.6 \\
802.000	& 802.250	& 7.8	& $\pm$ & 0.6 \\
802.250	& 802.500	& 8.0	& $\pm$ & 0.7 \\
802.500	& 802.700	& 8.1	& $\pm$ & 0.7 \\
802.700	& 802.950	& 7.8	& $\pm$ & 0.6 \\
802.950	& 803.200	& 8.1	& $\pm$ & 0.7 \\
803.200	& 803.400	& 8.1	& $\pm$ & 0.7 \\
803.400	& 803.650	& 8.0	& $\pm$ & 0.7 \\
803.650	& 803.900	& 7.8	& $\pm$ & 0.6 \\
803.900	& 804.200	& 7.9	& $\pm$ & 0.6 \\
804.200	& 804.400	& 8.0	& $\pm$ & 0.7 \\
804.400	& 804.650	& 8.0	& $\pm$ & 0.7 \\
804.650	& 804.900	& 8.0	& $\pm$ & 0.7 \\
804.900	& 805.100	& 8.1	& $\pm$ & 0.7 \\
805.100	& 805.350	& 8.2	& $\pm$ & 0.7 \\
805.350	& 805.600	& 8.2	& $\pm$ & 0.7 \\
805.600	& 805.800	& 8.2	& $\pm$ & 0.7 \\
805.800	& 806.050	& 8.2	& $\pm$ & 0.7 \\
806.050	& 806.300	& 8.2	& $\pm$ & 0.7 \\
806.300	& 806.500	& 8.1	& $\pm$ & 0.7 \\
806.500	& 806.750	& 7.9	& $\pm$ & 0.7 \\
806.750	& 807.100	& 7.9	& $\pm$ & 0.6 \\
807.100	& 807.300	& 7.9	& $\pm$ & 0.6 \\
807.300	& 807.550	& 7.9	& $\pm$ & 0.6 \\
807.550	& 807.800	& 7.9	& $\pm$ & 0.7 \\
807.800	& 808.000	& 7.8	& $\pm$ & 0.6 \\
808.000	& 808.250	& 7.8	& $\pm$ & 0.6 \\
808.250	& 808.500	& 7.7	& $\pm$ & 0.6 \\
808.500	& 808.700	& 7.7	& $\pm$ & 0.6 \\
808.700	& 808.950	& 7.7	& $\pm$ & 0.6 \\
808.950	& 809.200	& 7.7	& $\pm$ & 0.6 \\
809.200	& 809.400	& 7.7	& $\pm$ & 0.6 \\
809.400	& 809.650	& 7.7	& $\pm$ & 0.6 \\
809.650	& 809.900	& 7.7	& $\pm$ & 0.6 \\
809.900	& 810.100	& 7.7	& $\pm$ & 0.6 \\
810.100	& 810.350	& 7.8	& $\pm$ & 0.7 \\
810.350	& 810.600	& 7.7	& $\pm$ & 0.6 \\
810.600	& 810.800	& 7.8	& $\pm$ & 0.7 \\
810.800	& 811.050	& 7.7	& $\pm$ & 0.6 \\
811.050	& 811.250	& 7.7	& $\pm$ & 0.6 \\
811.250	& 811.500	& 7.7	& $\pm$ & 0.6 \\
811.500	& 811.750	& 7.9	& $\pm$ & 0.6 \\
811.750	& 811.950	& 7.8	& $\pm$ & 0.6 \\
811.950	& 812.200	& 7.9	& $\pm$ & 0.7 \\
812.200	& 812.400	& 7.8	& $\pm$ & 0.6 \\
812.400	& 812.650	& 7.7	& $\pm$ & 0.6 \\
812.650	& 812.900	& 7.8	& $\pm$ & 0.6 \\
812.900	& 813.100	& 7.8	& $\pm$ & 0.6 \\
813.100	& 813.350	& 7.9	& $\pm$ & 0.6 \\
813.350	& 813.550	& 7.9	& $\pm$ & 0.6 \\
813.550	& 813.800	& 7.8	& $\pm$ & 0.6 \\
813.800	& 814.200	& 7.8	& $\pm$ & 0.6 \\
814.200	& 814.400	& 7.9	& $\pm$ & 0.6 \\
814.400	& 814.650	& 7.9	& $\pm$ & 0.6 \\
814.650	& 814.850	& 8.0	& $\pm$ & 0.7 \\
814.850	& 815.100	& 8.0	& $\pm$ & 0.7 \\
815.100	& 815.350	& 7.9	& $\pm$ & 0.6 \\
815.350	& 815.550	& 7.9	& $\pm$ & 0.6 \\
815.550	& 815.800	& 7.8	& $\pm$ & 0.6 \\
815.800	& 816.000	& 7.8	& $\pm$ & 0.6 \\
816.000	& 816.250	& 7.8	& $\pm$ & 0.6 \\
816.250	& 816.450	& 7.8	& $\pm$ & 0.6 \\
816.450	& 816.700	& 7.9	& $\pm$ & 0.7 \\
816.700	& 816.900	& 7.8	& $\pm$ & 0.6 \\
816.900	& 817.150	& 7.8	& $\pm$ & 0.6 \\
817.150	& 817.400	& 7.9	& $\pm$ & 0.6 \\
817.400	& 817.600	& 8.0	& $\pm$ & 0.7 \\
817.600	& 817.850	& 8.1	& $\pm$ & 0.7 \\
817.850	& 818.050	& 7.9	& $\pm$ & 0.6 \\
818.050	& 818.300	& 7.9	& $\pm$ & 0.6 \\
818.300	& 818.500	& 7.9	& $\pm$ & 0.6 \\
818.500	& 818.750	& 7.9	& $\pm$ & 0.6 \\
818.750	& 818.950	& 7.8	& $\pm$ & 0.6 \\
818.950	& 819.200	& 7.8	& $\pm$ & 0.6 \\
819.200	& 819.400	& 7.8	& $\pm$ & 0.6 \\
819.400	& 819.650	& 7.8	& $\pm$ & 0.6 \\
819.650	& 819.850	& 7.8	& $\pm$ & 0.6 \\
819.850	& 820.100	& 7.8	& $\pm$ & 0.6 \\
820.100	& 820.350	& 7.8	& $\pm$ & 0.6 \\
820.350	& 820.550	& 7.8	& $\pm$ & 0.6 \\
820.550	& 820.800	& 7.8	& $\pm$ & 0.6 \\
820.800	& 821.000	& 7.8	& $\pm$ & 0.6 \\
821.000	& 821.250	& 7.8	& $\pm$ & 0.6 \\
821.250	& 821.450	& 8.0	& $\pm$ & 0.7 \\
821.450	& 821.700	& 7.8	& $\pm$ & 0.6 \\
821.700	& 821.900	& 7.8	& $\pm$ & 0.6 \\
821.900	& 822.150	& 7.8	& $\pm$ & 0.6 \\
822.150	& 822.350	& 7.8	& $\pm$ & 0.6 \\
822.350	& 822.600	& 7.9	& $\pm$ & 0.7 \\
822.600	& 822.800	& 7.8	& $\pm$ & 0.6 \\
822.800	& 823.050	& 7.8	& $\pm$ & 0.6 \\
823.050	& 823.250	& 7.8	& $\pm$ & 0.6 \\
823.250	& 823.500	& 7.8	& $\pm$ & 0.6 \\
823.500	& 823.700	& 7.8	& $\pm$ & 0.6 \\
823.700	& 823.900	& 7.8	& $\pm$ & 0.6 \\
823.900	& 824.150	& 7.8	& $\pm$ & 0.6 \\
824.150	& 824.350	& 7.8	& $\pm$ & 0.6 \\
824.350	& 824.600	& 7.8	& $\pm$ & 0.6 \\
824.600	& 824.800	& 7.9	& $\pm$ & 0.6 \\
824.800	& 825.050	& 8.0	& $\pm$ & 0.7 \\
825.050	& 825.250	& 7.9	& $\pm$ & 0.6 \\
825.250	& 825.500	& 7.9	& $\pm$ & 0.6 \\
825.500	& 825.700	& 7.9	& $\pm$ & 0.6 \\
825.700	& 825.950	& 7.8	& $\pm$ & 0.6 \\
825.950	& 826.150	& 7.8	& $\pm$ & 0.6 \\
826.150	& 826.450	& 7.8	& $\pm$ & 0.6 \\
826.450	& 826.650	& 7.8	& $\pm$ & 0.6 \\
826.650	& 826.900	& 7.8	& $\pm$ & 0.6 \\
826.900	& 827.100	& 7.8	& $\pm$ & 0.6 \\
827.100	& 827.300	& 7.8	& $\pm$ & 0.6 \\
827.300	& 827.550	& 7.8	& $\pm$ & 0.6 \\
827.550	& 827.750	& 7.8	& $\pm$ & 0.6 \\
827.750	& 828.000	& 8.0	& $\pm$ & 0.7 \\
828.000	& 828.200	& 7.9	& $\pm$ & 0.6 \\
828.200	& 828.450	& 7.8	& $\pm$ & 0.6 \\
828.450	& 828.650	& 7.8	& $\pm$ & 0.6 \\
828.650	& 828.850	& 7.9	& $\pm$ & 0.6 \\
828.850	& 829.100	& 7.8	& $\pm$ & 0.6 \\
829.100	& 829.300	& 7.8	& $\pm$ & 0.6 \\
829.300	& 829.550	& 7.9	& $\pm$ & 0.6 \\
829.550	& 829.750	& 7.8	& $\pm$ & 0.6 \\
829.750	& 830.000	& 7.9	& $\pm$ & 0.6 \\
830.000	& 830.200	& 7.8	& $\pm$ & 0.6 \\
830.200	& 830.400	& 7.9	& $\pm$ & 0.6 \\
830.400	& 830.650	& 7.9	& $\pm$ & 0.7 \\
830.650	& 830.850	& 7.9	& $\pm$ & 0.6 \\
830.850	& 831.100	& 7.8	& $\pm$ & 0.6 \\
831.100	& 831.300	& 7.9	& $\pm$ & 0.6 \\
831.300	& 831.500	& 8.0	& $\pm$ & 0.7 \\
831.500	& 831.750	& 7.9	& $\pm$ & 0.6 \\
831.750	& 831.950	& 7.9	& $\pm$ & 0.6 \\
831.950	& 832.200	& 7.8	& $\pm$ & 0.6 \\
832.200	& 832.400	& 7.8	& $\pm$ & 0.6 \\
832.400	& 832.650	& 7.8	& $\pm$ & 0.6 \\
832.650	& 832.900	& 7.9	& $\pm$ & 0.6 \\
832.900	& 833.100	& 7.9	& $\pm$ & 0.6 \\
833.100	& 833.300	& 7.9	& $\pm$ & 0.6 \\
833.300	& 833.550	& 7.9	& $\pm$ & 0.6 \\
833.550	& 833.750	& 7.9	& $\pm$ & 0.7 \\
833.750	& 834.000	& 7.9	& $\pm$ & 0.6 \\
834.000	& 834.200	& 8.0	& $\pm$ & 0.7 \\
834.200	& 834.400	& 7.9	& $\pm$ & 0.6 \\
834.400	& 834.650	& 7.9	& $\pm$ & 0.7 \\
834.650	& 834.850	& 7.9	& $\pm$ & 0.7 \\
834.850	& 835.050	& 8.0	& $\pm$ & 0.7 \\
835.050	& 835.300	& 8.0	& $\pm$ & 0.7 \\
835.300	& 835.500	& 8.1	& $\pm$ & 0.7 \\
835.500	& 835.700	& 8.2	& $\pm$ & 0.7 \\
835.700	& 835.950	& 8.3	& $\pm$ & 0.7 \\
835.950	& 836.150	& 8.2	& $\pm$ & 0.7 \\
836.150	& 836.400	& 8.4	& $\pm$ & 0.7 \\
836.400	& 836.600	& 8.4	& $\pm$ & 0.7 \\
836.600	& 836.800	& 8.7	& $\pm$ & 0.7 \\
836.800	& 837.050	& 8.8	& $\pm$ & 0.7 \\
837.050	& 837.250	& 8.9	& $\pm$ & 0.7 \\
837.250	& 837.450	& 8.8	& $\pm$ & 0.7 \\
837.450	& 837.700	& 8.7	& $\pm$ & 0.7 \\
837.700	& 837.900	& 8.5	& $\pm$ & 0.7 \\
837.900	& 838.100	& 8.6	& $\pm$ & 0.7 \\
838.100	& 838.350	& 8.3	& $\pm$ & 0.7 \\
838.350	& 838.550	& 8.4	& $\pm$ & 0.7 \\
838.550	& 838.750	& 8.2	& $\pm$ & 0.7 \\
838.750	& 839.000	& 8.2	& $\pm$ & 0.7 \\
839.000	& 839.200	& 8.1	& $\pm$ & 0.7 \\
839.200	& 839.400	& 8.1	& $\pm$ & 0.7 \\
839.400	& 839.600	& 8.1	& $\pm$ & 0.7 \\
839.600	& 839.850	& 8.1	& $\pm$ & 0.7 \\
839.850	& 840.050	& 8.1	& $\pm$ & 0.7 \\
840.050	& 840.250	& 8.1	& $\pm$ & 0.7 \\
840.250	& 840.500	& 8.1	& $\pm$ & 0.7 \\
840.500	& 840.700	& 8.2	& $\pm$ & 0.7 \\
840.700	& 840.900	& 8.3	& $\pm$ & 0.7 \\
840.900	& 841.150	& 8.4	& $\pm$ & 0.7 \\
841.150	& 841.350	& 8.2	& $\pm$ & 0.7 \\
841.350	& 841.550	& 8.0	& $\pm$ & 0.7 \\
841.550	& 841.800	& 8.1	& $\pm$ & 0.7 \\
841.800	& 842.150	& 8.1	& $\pm$ & 0.7 \\
842.150	& 842.350	& 8.0	& $\pm$ & 0.7 \\
842.350	& 842.550	& 8.1	& $\pm$ & 0.7 \\
842.550	& 842.800	& 8.0	& $\pm$ & 0.7 \\
842.800	& 843.000	& 8.1	& $\pm$ & 0.7 \\
843.000	& 843.200	& 8.1	& $\pm$ & 0.7 \\
843.200	& 843.400	& 8.0	& $\pm$ & 0.7 \\
843.400	& 843.650	& 8.0	& $\pm$ & 0.7 \\
843.650	& 843.850	& 8.0	& $\pm$ & 0.7 \\
843.850	& 844.050	& 8.0	& $\pm$ & 0.7 \\
844.050	& 844.300	& 8.0	& $\pm$ & 0.7 \\
844.300	& 844.600	& 8.0	& $\pm$ & 0.7 \\
844.600	& 844.800	& 8.0	& $\pm$ & 0.7 \\
844.800	& 845.000	& 8.0	& $\pm$ & 0.7 \\
845.000	& 845.250	& 8.1	& $\pm$ & 0.7 \\
845.250	& 845.450	& 8.2	& $\pm$ & 0.7 \\
845.450	& 845.650	& 8.1	& $\pm$ & 0.7 \\
845.650	& 845.850	& 8.1	& $\pm$ & 0.7 \\
845.850	& 846.100	& 8.0	& $\pm$ & 0.7 \\
846.100	& 846.300	& 8.3	& $\pm$ & 0.7 \\
846.300	& 846.500	& 8.1	& $\pm$ & 0.7 \\
846.500	& 846.700	& 8.1	& $\pm$ & 0.7 \\
846.700	& 846.950	& 8.1	& $\pm$ & 0.7 \\
846.950	& 847.150	& 8.2	& $\pm$ & 0.7 \\
847.150	& 847.350	& 8.1	& $\pm$ & 0.7 \\
847.350	& 847.550	& 8.1	& $\pm$ & 0.7 \\
847.550	& 847.800	& 8.2	& $\pm$ & 0.7 \\
847.800	& 848.000	& 8.2	& $\pm$ & 0.7 \\
848.000	& 848.200	& 8.2	& $\pm$ & 0.7 \\
848.200	& 848.400	& 8.3	& $\pm$ & 0.7 \\
848.400	& 848.600	& 8.2	& $\pm$ & 0.7 \\
848.600	& 848.850	& 8.3	& $\pm$ & 0.7 \\
848.850	& 849.050	& 8.2	& $\pm$ & 0.7 \\
849.050	& 849.250	& 8.2	& $\pm$ & 0.7 \\
849.250	& 849.450	& 8.2	& $\pm$ & 0.7 \\
849.450	& 849.650	& 8.2	& $\pm$ & 0.7 \\
849.650	& 849.900	& 8.2	& $\pm$ & 0.7 \\
849.900	& 850.100	& 8.2	& $\pm$ & 0.7 \\
850.100	& 850.300	& 8.2	& $\pm$ & 0.7 \\
850.300	& 850.500	& 8.2	& $\pm$ & 0.7 \\
850.500	& 850.750	& 8.2	& $\pm$ & 0.7 \\
850.750	& 850.950	& 8.2	& $\pm$ & 0.7 \\
850.950	& 851.150	& 8.2	& $\pm$ & 0.7 \\
851.150	& 851.350	& 8.1	& $\pm$ & 0.7 \\
851.350	& 851.550	& 8.1	& $\pm$ & 0.7 \\
851.550	& 851.800	& 8.1	& $\pm$ & 0.7 \\
851.800	& 852.000	& 8.2	& $\pm$ & 0.7 \\
852.000	& 852.200	& 8.2	& $\pm$ & 0.7 \\
852.200	& 852.400	& 8.3	& $\pm$ & 0.7 \\
852.400	& 852.600	& 8.1	& $\pm$ & 0.7 \\
852.600	& 852.800	& 8.2	& $\pm$ & 0.7 \\
852.800	& 853.050	& 8.1	& $\pm$ & 0.7 \\
853.050	& 853.250	& 8.2	& $\pm$ & 0.7 \\
853.250	& 853.450	& 8.1	& $\pm$ & 0.7 \\
853.450	& 853.650	& 8.3	& $\pm$ & 0.7 \\
853.650	& 853.850	& 8.2	& $\pm$ & 0.7 \\
853.850	& 854.050	& 8.2	& $\pm$ & 0.7 \\
854.050	& 854.300	& 8.2	& $\pm$ & 0.7 \\
854.300	& 854.500	& 8.2	& $\pm$ & 0.7 \\
854.500	& 854.700	& 8.3	& $\pm$ & 0.7 \\
854.700	& 854.900	& 8.2	& $\pm$ & 0.7 \\
854.900	& 855.100	& 8.2	& $\pm$ & 0.7 \\
855.100	& 855.300	& 8.2	& $\pm$ & 0.7 \\
855.300	& 855.550	& 8.3	& $\pm$ & 0.7 \\
855.550	& 855.750	& 8.2	& $\pm$ & 0.7 \\
855.750	& 855.950	& 8.2	& $\pm$ & 0.7 \\
855.950	& 856.150	& 8.3	& $\pm$ & 0.7 \\
856.150	& 856.350	& 8.2	& $\pm$ & 0.7 \\
856.350	& 856.550	& 8.2	& $\pm$ & 0.7 \\
856.550	& 856.750	& 8.3	& $\pm$ & 0.7 \\
856.750	& 857.000	& 8.3	& $\pm$ & 0.7 \\
857.000	& 857.200	& 8.3	& $\pm$ & 0.7 \\
857.200	& 857.400	& 8.4	& $\pm$ & 0.7 \\
857.400	& 857.600	& 8.3	& $\pm$ & 0.7 \\
857.600	& 857.800	& 8.3	& $\pm$ & 0.7 \\
857.800	& 858.000	& 8.4	& $\pm$ & 0.7 \\
858.000	& 858.200	& 8.3	& $\pm$ & 0.7 \\
858.200	& 858.450	& 8.4	& $\pm$ & 0.7 \\
858.450	& 858.650	& 8.4	& $\pm$ & 0.7 \\
858.650	& 858.850	& 8.5	& $\pm$ & 0.7 \\
858.850	& 859.050	& 8.6	& $\pm$ & 0.7 \\
859.050	& 859.250	& 8.5	& $\pm$ & 0.7 \\
859.250	& 859.450	& 8.4	& $\pm$ & 0.7 \\
859.450	& 859.650	& 8.6	& $\pm$ & 0.7 \\
859.650	& 859.850	& 8.5	& $\pm$ & 0.7 \\
859.850	& 860.100	& 8.4	& $\pm$ & 0.7 \\
860.100	& 860.300	& 8.6	& $\pm$ & 0.7 \\
860.300	& 860.500	& 8.5	& $\pm$ & 0.7 \\
860.500	& 860.700	& 8.4	& $\pm$ & 0.7 \\
860.700	& 860.900	& 8.6	& $\pm$ & 0.7 \\
860.900	& 861.100	& 8.5	& $\pm$ & 0.7 \\
861.100	& 861.300	& 8.5	& $\pm$ & 0.7 \\
861.300	& 861.500	& 8.6	& $\pm$ & 0.7 \\
861.500	& 861.700	& 8.6	& $\pm$ & 0.7 \\
861.700	& 861.900	& 8.5	& $\pm$ & 0.7 \\
861.900	& 862.150	& 8.5	& $\pm$ & 0.7 \\
862.150	& 862.350	& 8.8	& $\pm$ & 0.7 \\
862.350	& 862.550	& 8.7	& $\pm$ & 0.7 \\
862.550	& 862.750	& 8.6	& $\pm$ & 0.7 \\
862.750	& 862.950	& 8.5	& $\pm$ & 0.7 \\
862.950	& 863.150	& 8.5	& $\pm$ & 0.7 \\
863.150	& 863.350	& 8.5	& $\pm$ & 0.7 \\
863.350	& 863.550	& 8.7	& $\pm$ & 0.7 \\
863.550	& 863.750	& 8.5	& $\pm$ & 0.7 \\
863.750	& 863.950	& 8.5	& $\pm$ & 0.7 \\
863.950	& 864.150	& 8.7	& $\pm$ & 0.7 \\
864.150	& 864.350	& 8.6	& $\pm$ & 0.7 \\
864.350	& 864.550	& 8.5	& $\pm$ & 0.7 \\
864.550	& 864.800	& 8.7	& $\pm$ & 0.7 \\
864.800	& 865.000	& 8.5	& $\pm$ & 0.7 \\
865.000	& 865.200	& 8.5	& $\pm$ & 0.7 \\
865.200	& 865.400	& 8.6	& $\pm$ & 0.7 \\
865.400	& 865.600	& 8.6	& $\pm$ & 0.7 \\
865.600	& 865.800	& 8.6	& $\pm$ & 0.7 \\
865.800	& 866.000	& 8.7	& $\pm$ & 0.7 \\
866.000	& 866.200	& 8.9	& $\pm$ & 0.7 \\
866.200	& 866.400	& 9.1	& $\pm$ & 0.7 \\
866.400	& 866.600	& 9.3	& $\pm$ & 0.8 \\
866.600	& 866.800	& 9.3	& $\pm$ & 0.8 \\
866.800	& 867.000	& 9.1	& $\pm$ & 0.7 \\
867.000	& 867.200	& 8.9	& $\pm$ & 0.7 \\
867.200	& 867.400	& 8.8	& $\pm$ & 0.7 \\
867.400	& 867.600	& 8.7	& $\pm$ & 0.7 \\
867.600	& 867.800	& 8.6	& $\pm$ & 0.7 \\
867.800	& 868.000	& 8.6	& $\pm$ & 0.7 \\
868.000	& 868.200	& 8.6	& $\pm$ & 0.7 \\
868.200	& 868.400	& 8.6	& $\pm$ & 0.7 \\
868.400	& 868.600	& 8.5	& $\pm$ & 0.7 \\
868.600	& 868.800	& 8.5	& $\pm$ & 0.7 \\
868.800	& 871.000	& 8.5	& $\pm$ & 0.7 \\
871.000	& 871.350	& 8.5	& $\pm$ & 0.7 \\
871.350	& 871.550	& 8.5	& $\pm$ & 0.7 \\
871.550	& 871.750	& 8.6	& $\pm$ & 0.7 \\
871.750	& 871.950	& 8.6	& $\pm$ & 0.7 \\
871.950	& 872.150	& 8.6	& $\pm$ & 0.7 \\
872.150	& 872.350	& 8.5	& $\pm$ & 0.7 \\
872.350	& 872.550	& 8.6	& $\pm$ & 0.7 \\
872.550	& 872.750	& 8.6	& $\pm$ & 0.7 \\
872.750	& 872.950	& 8.6	& $\pm$ & 0.7 \\
872.950	& 873.150	& 8.7	& $\pm$ & 0.7 \\
873.150	& 873.350	& 8.7	& $\pm$ & 0.7 \\
873.350	& 873.550	& 8.7	& $\pm$ & 0.7 \\
873.550	& 873.750	& 8.8	& $\pm$ & 0.7 \\
873.750	& 873.950	& 8.7	& $\pm$ & 0.7 \\
873.950	& 874.150	& 8.7	& $\pm$ & 0.7 \\
874.150	& 874.350	& 8.7	& $\pm$ & 0.7 \\
874.350	& 874.550	& 8.7	& $\pm$ & 0.7 \\
874.550	& 874.750	& 8.7	& $\pm$ & 0.7 \\
874.750	& 874.950	& 8.8	& $\pm$ & 0.7 \\
874.950	& 875.150	& 8.8	& $\pm$ & 0.7 \\
875.150	& 875.350	& 8.9	& $\pm$ & 0.7 \\
875.350	& 875.550	& 9.0	& $\pm$ & 0.7 \\
875.550	& 875.750	& 8.9	& $\pm$ & 0.7 \\
875.750	& 875.950	& 8.8	& $\pm$ & 0.7 \\
875.950	& 876.150	& 8.7	& $\pm$ & 0.7 \\
876.150	& 876.350	& 8.7	& $\pm$ & 0.7 \\
876.350	& 876.550	& 8.8	& $\pm$ & 0.7 \\
876.550	& 876.750	& 8.6	& $\pm$ & 0.7 \\
876.750	& 876.950	& 8.6	& $\pm$ & 0.7 \\
876.950	& 877.150	& 8.7	& $\pm$ & 0.7 \\
877.150	& 877.350	& 8.7	& $\pm$ & 0.7 \\
877.350	& 877.550	& 8.6	& $\pm$ & 0.7 \\
877.550	& 877.750	& 8.6	& $\pm$ & 0.7 \\
877.750	& 877.950	& 8.6	& $\pm$ & 0.7 \\
877.950	& 878.150	& 8.6	& $\pm$ & 0.7 \\
878.150	& 878.350	& 8.6	& $\pm$ & 0.7 \\
878.350	& 878.500	& 8.6	& $\pm$ & 0.7 \\
878.500	& 878.700	& 8.6	& $\pm$ & 0.7 \\
878.700	& 878.900	& 8.6	& $\pm$ & 0.7 \\
878.900	& 879.100	& 8.6	& $\pm$ & 0.7 \\
879.100	& 879.300	& 8.6	& $\pm$ & 0.7 \\
879.300	& 879.500	& 8.6	& $\pm$ & 0.7 \\
879.500	& 879.700	& 8.6	& $\pm$ & 0.7 \\
879.700	& 879.900	& 8.6	& $\pm$ & 0.7 \\
879.900	& 880.100	& 8.6	& $\pm$ & 0.7 \\
880.100	& 880.300	& 8.7	& $\pm$ & 0.7 \\
880.300	& 880.500	& 8.7	& $\pm$ & 0.7 \\
880.500	& 880.700	& 8.7	& $\pm$ & 0.7 \\
880.700	& 880.900	& 8.6	& $\pm$ & 0.7 \\
880.900	& 881.100	& 8.6	& $\pm$ & 0.7 \\
881.100	& 881.250	& 8.7	& $\pm$ & 0.7 \\
881.250	& 881.450	& 8.7	& $\pm$ & 0.7 \\
881.450	& 881.650	& 8.8	& $\pm$ & 0.7 \\
881.650	& 881.850	& 8.6	& $\pm$ & 0.7 \\
881.850	& 882.050	& 8.6	& $\pm$ & 0.7 \\
882.050	& 882.250	& 8.6	& $\pm$ & 0.7 \\
882.250	& 882.450	& 8.6	& $\pm$ & 0.7 \\
882.450	& 882.650	& 8.7	& $\pm$ & 0.7 \\
882.650	& 882.850	& 8.7	& $\pm$ & 0.7 \\
882.850	& 883.050	& 8.7	& $\pm$ & 0.7 \\
883.050	& 883.200	& 8.7	& $\pm$ & 0.7 \\
883.200	& 883.400	& 8.7	& $\pm$ & 0.7 \\
883.400	& 883.600	& 8.7	& $\pm$ & 0.7 \\
883.600	& 883.800	& 8.9	& $\pm$ & 0.7 \\
883.800	& 884.000	& 8.8	& $\pm$ & 0.7 \\
884.000	& 884.200	& 8.8	& $\pm$ & 0.7 \\
884.200	& 884.400	& 8.7	& $\pm$ & 0.7 \\
884.400	& 884.600	& 8.9	& $\pm$ & 0.7 \\
884.600	& 884.800	& 8.7	& $\pm$ & 0.7 \\
884.800	& 885.000	& 8.7	& $\pm$ & 0.7 \\
885.000	& 885.150	& 8.7	& $\pm$ & 0.7 \\
885.150	& 885.350	& 8.8	& $\pm$ & 0.7 \\
885.350	& 885.550	& 8.8	& $\pm$ & 0.7 \\
885.550	& 885.750	& 8.7	& $\pm$ & 0.7 \\
885.750	& 885.950	& 8.7	& $\pm$ & 0.7 \\
885.950	& 886.150	& 8.8	& $\pm$ & 0.7 \\
886.150	& 886.350	& 8.6	& $\pm$ & 0.7 \\
886.350	& 886.550	& 8.7	& $\pm$ & 0.7 \\
886.550	& 886.700	& 8.8	& $\pm$ & 0.7 \\
886.700	& 886.900	& 8.7	& $\pm$ & 0.7 \\
886.900	& 887.100	& 8.7	& $\pm$ & 0.7 \\
887.100	& 887.300	& 8.7	& $\pm$ & 0.7 \\
887.300	& 887.500	& 8.7	& $\pm$ & 0.7 \\
887.500	& 887.700	& 8.9	& $\pm$ & 0.7 \\
887.700	& 887.900	& 8.7	& $\pm$ & 0.7 \\
887.900	& 888.050	& 8.7	& $\pm$ & 0.7 \\
888.050	& 888.250	& 8.8	& $\pm$ & 0.7 \\
888.250	& 888.450	& 8.9	& $\pm$ & 0.7 \\
888.450	& 888.650	& 8.8	& $\pm$ & 0.7 \\
888.650	& 888.850	& 8.8	& $\pm$ & 0.7 \\
888.850	& 889.050	& 8.7	& $\pm$ & 0.7 \\
889.050	& 889.250	& 8.7	& $\pm$ & 0.7 \\
889.250	& 889.400	& 8.7	& $\pm$ & 0.7 \\
889.400	& 889.600	& 8.7	& $\pm$ & 0.7 \\
889.600	& 889.800	& 8.9	& $\pm$ & 0.7 \\
889.800	& 890.000	& 8.8	& $\pm$ & 0.7 \\
890.000	& 890.200	& 9.3	& $\pm$ & 0.8 \\
890.200	& 890.400	& 9.5	& $\pm$ & 0.8 \\
890.400	& 890.550	& 9.2	& $\pm$ & 0.8 \\
890.550	& 890.750	& 8.9	& $\pm$ & 0.7 \\
890.750	& 890.950	& 8.6	& $\pm$ & 0.7 \\
890.950	& 891.150	& 8.6	& $\pm$ & 0.7 \\
891.150	& 891.350	& 8.8	& $\pm$ & 0.7 \\
891.350	& 891.550	& 8.8	& $\pm$ & 0.7 \\
891.550	& 891.700	& 8.7	& $\pm$ & 0.7 \\
891.700	& 891.900	& 8.6	& $\pm$ & 0.7 \\
891.900	& 892.100	& 8.6	& $\pm$ & 0.7 \\
892.100	& 892.300	& 8.7	& $\pm$ & 0.7 \\
892.300	& 892.500	& 8.6	& $\pm$ & 0.7 \\
892.500	& 892.650	& 8.7	& $\pm$ & 0.7 \\
892.650	& 892.850	& 8.5	& $\pm$ & 0.7 \\
892.850	& 893.050	& 8.6	& $\pm$ & 0.7 \\
893.050	& 893.250	& 8.6	& $\pm$ & 0.7 \\
893.250	& 893.450	& 8.7	& $\pm$ & 0.7 \\
893.450	& 893.600	& 8.7	& $\pm$ & 0.7 \\
893.600	& 893.800	& 8.6	& $\pm$ & 0.7 \\
893.800	& 894.000	& 8.5	& $\pm$ & 0.7 \\
894.000	& 894.200	& 8.5	& $\pm$ & 0.7 \\
894.200	& 894.400	& 8.5	& $\pm$ & 0.7 \\
894.400	& 894.600	& 8.7	& $\pm$ & 0.7 \\
894.600	& 894.750	& 8.6	& $\pm$ & 0.7 \\
894.750	& 894.950	& 8.6	& $\pm$ & 0.7 \\
894.950	& 895.150	& 8.6	& $\pm$ & 0.7 \\
895.150	& 895.350	& 8.6	& $\pm$ & 0.7 \\
895.350	& 895.500	& 8.7	& $\pm$ & 0.7 \\
895.500	& 896.100	& 8.8	& $\pm$ & 0.7 \\
896.100	& 896.300	& 8.9	& $\pm$ & 0.7 \\
896.300	& 896.500	& 8.9	& $\pm$ & 0.7 \\
896.500	& 896.700	& 8.8	& $\pm$ & 0.7 \\
896.700	& 896.850	& 8.6	& $\pm$ & 0.7 \\
896.850	& 897.050	& 8.6	& $\pm$ & 0.7 \\
897.050	& 898.500	& 8.8	& $\pm$ & 0.7 \\
898.500	& 898.700	& 8.7	& $\pm$ & 0.7 \\
898.700	& 898.850	& 8.7	& $\pm$ & 0.7 \\
898.850	& 899.050	& 8.6	& $\pm$ & 0.7 \\
899.050	& 899.250	& 8.6	& $\pm$ & 0.7 \\
899.250	& 899.450	& 8.8	& $\pm$ & 0.7 \\
899.450	& 899.650	& 8.9	& $\pm$ & 0.8 \\
899.650	& 899.800	& 8.7	& $\pm$ & 0.7 \\
899.800	& 900.000	& 8.6	& $\pm$ & 0.7 \\
900.000	& 900.200	& 8.6	& $\pm$ & 0.7 \\
900.200	& 900.400	& 8.7	& $\pm$ & 0.7 \\
900.400	& 900.550	& 8.9	& $\pm$ & 0.7 \\
900.550	& 900.750	& 9.0	& $\pm$ & 0.7 \\
900.750	& 900.950	& 8.6	& $\pm$ & 0.7 \\
900.950	& 901.150	& 8.7	& $\pm$ & 0.7 \\
901.150	& 901.300	& 8.7	& $\pm$ & 0.7 \\
901.300	& 901.500	& 8.7	& $\pm$ & 0.7 \\
901.500	& 901.700	& 8.7	& $\pm$ & 0.7 \\
901.700	& 901.850	& 8.8	& $\pm$ & 0.7 \\
901.850	& 902.050	& 8.7	& $\pm$ & 0.7 \\
902.050	& 902.250	& 8.7	& $\pm$ & 0.7 \\
902.250	& 902.450	& 8.8	& $\pm$ & 0.7 \\
902.450	& 902.600	& 8.8	& $\pm$ & 0.7 \\
902.600	& 902.800	& 8.9	& $\pm$ & 0.7 \\
902.800	& 903.000	& 8.9	& $\pm$ & 0.7 \\
903.000	& 903.200	& 9.0	& $\pm$ & 0.8 \\
903.200	& 903.350	& 8.8	& $\pm$ & 0.7 \\
903.350	& 903.550	& 8.8	& $\pm$ & 0.7 \\
903.550	& 903.750	& 8.9	& $\pm$ & 0.7 \\
903.750	& 903.950	& 8.8	& $\pm$ & 0.7 \\
903.950	& 904.100	& 8.8	& $\pm$ & 0.7 \\
904.100	& 904.300	& 8.9	& $\pm$ & 0.7 \\
904.300	& 904.500	& 8.9	& $\pm$ & 0.7 \\
904.500	& 904.650	& 8.8	& $\pm$ & 0.7 \\
904.650	& 904.850	& 8.8	& $\pm$ & 0.7 \\
904.850	& 905.050	& 8.8	& $\pm$ & 0.7 \\
905.050	& 905.250	& 8.8	& $\pm$ & 0.7 \\
905.250	& 905.400	& 8.9	& $\pm$ & 0.7 \\
905.400	& 905.600	& 9.0	& $\pm$ & 0.7 \\
905.600	& 905.800	& 9.4	& $\pm$ & 0.8 \\
905.800	& 905.950	& 9.1	& $\pm$ & 0.7 \\
905.950	& 906.150	& 9.3	& $\pm$ & 0.8 \\
906.150	& 906.350	& 9.1	& $\pm$ & 0.7 \\
906.350	& 906.500	& 9.1	& $\pm$ & 0.7 \\
906.500	& 906.700	& 8.9	& $\pm$ & 0.7 \\
906.700	& 906.900	& 8.9	& $\pm$ & 0.7 \\
906.900	& 907.100	& 9.0	& $\pm$ & 0.7 \\
907.100	& 907.250	& 9.1	& $\pm$ & 0.7 \\
907.250	& 907.450	& 9.1	& $\pm$ & 0.7 \\
907.450	& 907.650	& 9.1	& $\pm$ & 0.7 \\
907.650	& 907.800	& 9.1	& $\pm$ & 0.7 \\
907.800	& 908.000	& 9.1	& $\pm$ & 0.7 \\
908.000	& 908.200	& 8.9	& $\pm$ & 0.7 \\
908.200	& 908.350	& 8.9	& $\pm$ & 0.7 \\
908.350	& 908.550	& 8.9	& $\pm$ & 0.7 \\
908.550	& 908.750	& 9.0	& $\pm$ & 0.7 \\
908.750	& 908.900	& 8.9	& $\pm$ & 0.7 \\
908.900	& 909.100	& 8.8	& $\pm$ & 0.7 \\
909.100	& 909.300	& 9.0	& $\pm$ & 0.7 \\
909.300	& 909.450	& 8.9	& $\pm$ & 0.7 \\
909.450	& 909.650	& 9.2	& $\pm$ & 0.8 \\
909.650	& 909.850	& 9.1	& $\pm$ & 0.8 \\
909.850	& 910.000	& 8.9	& $\pm$ & 0.7 \\
910.000	& 910.200	& 8.8	& $\pm$ & 0.7 \\
910.200	& 910.400	& 8.8	& $\pm$ & 0.7 \\
910.400	& 910.600	& 8.9	& $\pm$ & 0.7 \\
910.600	& 910.750	& 8.7	& $\pm$ & 0.7 \\
910.750	& 910.950	& 8.7	& $\pm$ & 0.7 \\
910.950	& 911.100	& 8.6	& $\pm$ & 0.7 \\
911.100	& 911.300	& 8.7	& $\pm$ & 0.7 \\
911.300	& 911.500	& 8.8	& $\pm$ & 0.7 \\
911.500	& 911.650	& 8.8	& $\pm$ & 0.7 \\
911.650	& 911.850	& 8.7	& $\pm$ & 0.7 \\
911.850	& 912.050	& 8.6	& $\pm$ & 0.7 \\
912.050	& 912.200	& 8.7	& $\pm$ & 0.7 \\
912.200	& 912.400	& 8.8	& $\pm$ & 0.7 \\
912.400	& 912.600	& 8.7	& $\pm$ & 0.7 \\
912.600	& 912.750	& 8.6	& $\pm$ & 0.7 \\
912.750	& 912.950	& 8.7	& $\pm$ & 0.7 \\
912.950	& 913.150	& 8.7	& $\pm$ & 0.7 \\
913.150	& 913.300	& 8.7	& $\pm$ & 0.7 \\
913.300	& 913.500	& 8.8	& $\pm$ & 0.7 \\
913.500	& 913.700	& 8.6	& $\pm$ & 0.7 \\
913.700	& 913.850	& 8.8	& $\pm$ & 0.7 \\
913.850	& 914.050	& 8.7	& $\pm$ & 0.7 \\
914.050	& 914.250	& 8.8	& $\pm$ & 0.7 \\
914.250	& 914.400	& 8.7	& $\pm$ & 0.7 \\
914.400	& 914.600	& 8.6	& $\pm$ & 0.7 \\
914.600	& 914.750	& 8.6	& $\pm$ & 0.7 \\
914.750	& 914.950	& 8.6	& $\pm$ & 0.7 \\
914.950	& 915.150	& 8.6	& $\pm$ & 0.7 \\
915.150	& 915.300	& 8.6	& $\pm$ & 0.7 \\
915.300	& 915.500	& 8.8	& $\pm$ & 0.7 \\
915.500	& 915.700	& 8.7	& $\pm$ & 0.7 \\
915.700	& 915.850	& 8.7	& $\pm$ & 0.7 \\
915.850	& 916.050	& 8.7	& $\pm$ & 0.7 \\
916.050	& 916.200	& 8.8	& $\pm$ & 0.7 \\
916.200	& 916.400	& 8.8	& $\pm$ & 0.7 \\
916.400	& 916.600	& 8.8	& $\pm$ & 0.7 \\
916.600	& 916.750	& 8.7	& $\pm$ & 0.7 \\
916.750	& 916.950	& 8.7	& $\pm$ & 0.7 \\
916.950	& 917.150	& 8.7	& $\pm$ & 0.7 \\
917.150	& 917.300	& 8.8	& $\pm$ & 0.7 \\
917.300	& 917.500	& 9.0	& $\pm$ & 0.8 \\
917.500	& 917.650	& 9.1	& $\pm$ & 0.8 \\
917.650	& 917.850	& 9.1	& $\pm$ & 0.8 \\
917.850	& 918.050	& 8.8	& $\pm$ & 0.7 \\
918.050	& 918.200	& 9.1	& $\pm$ & 0.8 \\
918.200	& 918.400	& 8.8	& $\pm$ & 0.7 \\
918.400	& 918.550	& 8.8	& $\pm$ & 0.7 \\
918.550	& 918.750	& 8.8	& $\pm$ & 0.7 \\
918.750	& 918.950	& 8.8	& $\pm$ & 0.7 \\
918.950	& 919.100	& 8.7	& $\pm$ & 0.7 \\
919.100	& 919.300	& 8.9	& $\pm$ & 0.7 \\
919.300	& 919.450	& 9.1	& $\pm$ & 0.8 \\
919.450	& 919.650	& 9.6	& $\pm$ & 0.8 \\
919.650	& 919.850	& 9.0	& $\pm$ & 0.7 \\
919.850	& 920.000	& 8.8	& $\pm$ & 0.7 \\
920.000	& 920.200	& 8.7	& $\pm$ & 0.7 \\
920.200	& 920.350	& 8.7	& $\pm$ & 0.7 \\
920.350	& 922.400	& 8.7	& $\pm$ & 0.7 \\
922.400	& 922.600	& 8.7	& $\pm$ & 0.7 \\
922.600	& 922.750	& 8.7	& $\pm$ & 0.7 \\
922.750	& 922.950	& 8.7	& $\pm$ & 0.7 \\
922.950	& 923.100	& 8.7	& $\pm$ & 0.7 \\
923.100	& 923.300	& 8.7	& $\pm$ & 0.7 \\
923.300	& 923.450	& 8.7	& $\pm$ & 0.7 \\
923.450	& 923.650	& 8.7	& $\pm$ & 0.7 \\
923.650	& 923.850	& 8.7	& $\pm$ & 0.7 \\
923.850	& 924.000	& 8.7	& $\pm$ & 0.7 \\
924.000	& 924.200	& 8.7	& $\pm$ & 0.7 \\
924.200	& 924.350	& 8.7	& $\pm$ & 0.7 \\
924.350	& 924.650	& 8.7	& $\pm$ & 0.7 \\
924.650	& 924.800	& 8.7	& $\pm$ & 0.7 \\
924.800	& 925.000	& 8.9	& $\pm$ & 0.7 \\
925.000	& 925.150	& 8.7	& $\pm$ & 0.7 \\
925.150	& 925.400	& 8.7	& $\pm$ & 0.7 \\
925.400	& 926.600	& 8.8	& $\pm$ & 0.7 \\
926.600	& 926.750	& 8.7	& $\pm$ & 0.7 \\
926.750	& 926.950	& 8.7	& $\pm$ & 0.7 \\
926.950	& 927.100	& 8.7	& $\pm$ & 0.7 \\
927.100	& 927.300	& 8.8	& $\pm$ & 0.7 \\
927.300	& 927.450	& 8.8	& $\pm$ & 0.7 \\
927.450	& 927.650	& 8.8	& $\pm$ & 0.7 \\
927.650	& 927.800	& 8.9	& $\pm$ & 0.7 \\
927.800	& 928.400	& 8.9	& $\pm$ & 0.7 \\
928.400	& 928.550	& 9.1	& $\pm$ & 0.7 \\
928.550	& 928.750	& 9.2	& $\pm$ & 0.8 \\
928.750	& 928.900	& 9.1	& $\pm$ & 0.7 \\
928.900	& 929.100	& 9.1	& $\pm$ & 0.7 \\
929.100	& 929.250	& 9.0	& $\pm$ & 0.7 \\
929.250	& 929.450	& 9.0	& $\pm$ & 0.7 \\
929.450	& 929.600	& 9.0	& $\pm$ & 0.7 \\
929.600	& 929.800	& 9.1	& $\pm$ & 0.7 \\
929.800	& 930.000	& 9.1	& $\pm$ & 0.7 \\
930.000	& 930.150	& 9.2	& $\pm$ & 0.8 \\
930.150	& 930.350	& 9.4	& $\pm$ & 0.8 \\
930.350	& 930.500	& 10.2	& $\pm$ & 0.8 \\
930.500	& 930.700	& 10.9	& $\pm$ & 0.9 \\
930.700	& 930.850	& 11.2	& $\pm$ & 0.9 \\
930.850	& 931.050	& 10.3	& $\pm$ & 0.8 \\
931.050	& 931.200	& 11.0	& $\pm$ & 0.9 \\
931.200	& 931.500	& 11.0	& $\pm$ & 0.9 \\
931.500	& 931.650	& 10.2	& $\pm$ & 0.8 \\
931.650	& 931.850	& 9.7	& $\pm$ & 0.8 \\
931.850	& 932.000	& 9.6	& $\pm$ & 0.8 \\
932.000	& 932.200	& 9.6	& $\pm$ & 0.8 \\
932.200	& 932.350	& 9.3	& $\pm$ & 0.8 \\
932.350	& 932.550	& 9.2	& $\pm$ & 0.8 \\
932.550	& 932.700	& 9.1	& $\pm$ & 0.7 \\
932.700	& 932.900	& 9.1	& $\pm$ & 0.7 \\
932.900	& 933.050	& 9.1	& $\pm$ & 0.7 \\
933.050	& 933.250	& 9.1	& $\pm$ & 0.7 \\
933.250	& 933.400	& 9.3	& $\pm$ & 0.8 \\
933.400	& 933.600	& 9.1	& $\pm$ & 0.7 \\
933.600	& 933.750	& 9.0	& $\pm$ & 0.7 \\
933.750	& 933.950	& 8.9	& $\pm$ & 0.7 \\
933.950	& 934.100	& 8.9	& $\pm$ & 0.7 \\
934.100	& 934.300	& 8.9	& $\pm$ & 0.7 \\
934.300	& 934.450	& 8.9	& $\pm$ & 0.7 \\
934.450	& 934.600	& 8.9	& $\pm$ & 0.7 \\
934.600	& 934.800	& 8.9	& $\pm$ & 0.7 \\
934.800	& 934.950	& 8.9	& $\pm$ & 0.7 \\
934.950	& 935.150	& 8.9	& $\pm$ & 0.7 \\
935.150	& 935.300	& 9.0	& $\pm$ & 0.8 \\
935.300	& 935.500	& 8.9	& $\pm$ & 0.7 \\
935.500	& 935.650	& 8.9	& $\pm$ & 0.7 \\
935.650	& 935.850	& 8.9	& $\pm$ & 0.7 \\
935.850	& 936.000	& 8.9	& $\pm$ & 0.7 \\
936.000	& 936.200	& 9.0	& $\pm$ & 0.7 \\
936.200	& 936.350	& 9.0	& $\pm$ & 0.7 \\
936.350	& 936.550	& 9.0	& $\pm$ & 0.7 \\
936.550	& 936.700	& 9.0	& $\pm$ & 0.7 \\
936.700	& 936.900	& 9.2	& $\pm$ & 0.8 \\
936.900	& 937.050	& 9.0	& $\pm$ & 0.7 \\
937.050	& 937.250	& 9.0	& $\pm$ & 0.7 \\
937.250	& 937.400	& 9.1	& $\pm$ & 0.8 \\
937.400	& 937.550	& 9.1	& $\pm$ & 0.8 \\
937.550	& 937.750	& 9.0	& $\pm$ & 0.7 \\
937.750	& 937.900	& 9.1	& $\pm$ & 0.7 \\
937.900	& 938.100	& 9.6	& $\pm$ & 0.8 \\
938.100	& 938.250	& 10.3	& $\pm$ & 0.8 \\
938.250	& 938.450	& 9.5	& $\pm$ & 0.8 \\
938.450	& 938.600	& 9.2	& $\pm$ & 0.8 \\
938.600	& 938.800	& 9.0	& $\pm$ & 0.7 \\
938.800	& 938.950	& 9.0	& $\pm$ & 0.7 \\
938.950	& 939.150	& 9.1	& $\pm$ & 0.7 \\
939.150	& 939.300	& 9.1	& $\pm$ & 0.7 \\
939.300	& 939.450	& 9.0	& $\pm$ & 0.7 \\
939.450	& 939.650	& 9.1	& $\pm$ & 0.7 \\
939.650	& 939.800	& 9.2	& $\pm$ & 0.8 \\
939.800	& 940.000	& 9.2	& $\pm$ & 0.8 \\
940.000	& 940.150	& 9.2	& $\pm$ & 0.8 \\
940.150	& 940.350	& 9.1	& $\pm$ & 0.7 \\
940.350	& 940.500	& 9.1	& $\pm$ & 0.7 \\
940.500	& 940.700	& 9.1	& $\pm$ & 0.8 \\
940.700	& 940.850	& 9.3	& $\pm$ & 0.8 \\
940.850	& 941.000	& 9.1	& $\pm$ & 0.7 \\
941.000	& 941.200	& 9.2	& $\pm$ & 0.8 \\
941.200	& 941.350	& 9.3	& $\pm$ & 0.8 \\
941.350	& 941.550	& 9.3	& $\pm$ & 0.8 \\
941.550	& 941.700	& 9.3	& $\pm$ & 0.8 \\
941.700	& 941.900	& 9.5	& $\pm$ & 0.8 \\
941.900	& 942.050	& 9.6	& $\pm$ & 0.8 \\
942.050	& 942.200	& 9.7	& $\pm$ & 0.8 \\
942.200	& 942.400	& 9.8	& $\pm$ & 0.8 \\
942.400	& 942.550	& 10.3	& $\pm$ & 0.8 \\
942.550	& 942.750	& 11.2	& $\pm$ & 0.9 \\
942.750	& 942.900	& 11.0	& $\pm$ & 0.9 \\
942.900	& 943.050	& 10.2	& $\pm$ & 0.8 \\
943.050	& 943.250	& 9.7	& $\pm$ & 0.8 \\
943.250	& 943.400	& 9.6	& $\pm$ & 0.8 \\
943.400	& 943.600	& 9.6	& $\pm$ & 0.8 \\
943.600	& 943.750	& 9.5	& $\pm$ & 0.8 \\
943.750	& 943.950	& 9.6	& $\pm$ & 0.8 \\
943.950	& 944.100	& 9.3	& $\pm$ & 0.8 \\
944.100	& 944.250	& 9.2	& $\pm$ & 0.8 \\
944.250	& 944.450	& 9.1	& $\pm$ & 0.7 \\
944.450	& 944.600	& 9.1	& $\pm$ & 0.7 \\
944.600	& 944.800	& 9.1	& $\pm$ & 0.7 \\
944.800	& 944.950	& 9.1	& $\pm$ & 0.7 \\
944.950	& 945.100	& 9.2	& $\pm$ & 0.8 \\
945.100	& 945.300	& 9.0	& $\pm$ & 0.7 \\
945.300	& 945.450	& 9.0	& $\pm$ & 0.7 \\
945.450	& 945.650	& 9.0	& $\pm$ & 0.7 \\
945.650	& 945.800	& 9.1	& $\pm$ & 0.7 \\
945.800	& 945.950	& 9.0	& $\pm$ & 0.7 \\
945.950	& 946.150	& 9.0	& $\pm$ & 0.7 \\
946.150	& 946.300	& 9.0	& $\pm$ & 0.7 \\
946.300	& 946.500	& 9.0	& $\pm$ & 0.7 \\
946.500	& 946.650	& 9.0	& $\pm$ & 0.7 \\
946.650	& 946.800	& 9.0	& $\pm$ & 0.7 \\
946.800	& 947.000	& 8.9	& $\pm$ & 0.7 \\
947.000	& 947.150	& 8.9	& $\pm$ & 0.7 \\
947.150	& 947.350	& 8.9	& $\pm$ & 0.7 \\
947.350	& 947.500	& 8.9	& $\pm$ & 0.7 \\
947.500	& 947.650	& 8.9	& $\pm$ & 0.7 \\
947.650	& 947.850	& 8.9	& $\pm$ & 0.7 \\
947.850	& 948.000	& 8.9	& $\pm$ & 0.7 \\
948.000	& 948.150	& 8.9	& $\pm$ & 0.7 \\
948.150	& 948.350	& 8.9	& $\pm$ & 0.7 \\
948.350	& 948.500	& 8.9	& $\pm$ & 0.7 \\
948.500	& 948.700	& 8.9	& $\pm$ & 0.7 \\
948.700	& 948.850	& 9.0	& $\pm$ & 0.7 \\
948.850	& 949.000	& 8.9	& $\pm$ & 0.7 \\
949.000	& 949.200	& 9.0	& $\pm$ & 0.7 \\
949.200	& 949.350	& 9.0	& $\pm$ & 0.7 \\
949.350	& 949.550	& 9.1	& $\pm$ & 0.8 \\
949.550	& 949.700	& 9.0	& $\pm$ & 0.7 \\
949.700	& 949.850	& 9.2	& $\pm$ & 0.8 \\
949.850	& 950.050	& 9.0	& $\pm$ & 0.7 \\
950.050	& 950.200	& 9.2	& $\pm$ & 0.8 \\
950.200	& 950.350	& 9.1	& $\pm$ & 0.7 \\
950.350	& 950.550	& 9.1	& $\pm$ & 0.7 \\
950.550	& 950.700	& 9.0	& $\pm$ & 0.7 \\
950.700	& 950.850	& 9.1	& $\pm$ & 0.7 \\
950.850	& 951.250	& 9.0	& $\pm$ & 0.7 \\
951.250	& 951.550	& 9.0	& $\pm$ & 0.7 \\
951.550	& 951.850	& 9.0	& $\pm$ & 0.7 \\
951.850	& 952.000	& 9.2	& $\pm$ & 0.8 \\
952.000	& 952.150	& 9.0	& $\pm$ & 0.7 \\
952.150	& 952.350	& 9.3	& $\pm$ & 0.8 \\
952.350	& 952.500	& 9.0	& $\pm$ & 0.7 \\
952.500	& 952.650	& 9.0	& $\pm$ & 0.7 \\
952.650	& 952.850	& 9.1	& $\pm$ & 0.7 \\
952.850	& 953.000	& 9.1	& $\pm$ & 0.7 \\
953.000	& 953.150	& 9.1	& $\pm$ & 0.7 \\
953.150	& 953.350	& 9.1	& $\pm$ & 0.7 \\
953.350	& 953.500	& 9.3	& $\pm$ & 0.8 \\
953.500	& 953.650	& 9.8	& $\pm$ & 0.8 \\
953.650	& 953.850	& 9.6	& $\pm$ & 0.8 \\
953.850	& 954.400	& 9.2	& $\pm$ & 0.8 \\
954.400	& 954.550	& 9.1	& $\pm$ & 0.7 \\
954.550	& 954.750	& 9.1	& $\pm$ & 0.7 \\
954.750	& 954.900	& 9.1	& $\pm$ & 0.7 \\
954.900	& 955.050	& 9.1	& $\pm$ & 0.7 \\
955.050	& 955.250	& 9.1	& $\pm$ & 0.7 \\
955.250	& 955.400	& 9.2	& $\pm$ & 0.8 \\
955.400	& 955.550	& 9.1	& $\pm$ & 0.7 \\
955.550	& 955.750	& 9.1	& $\pm$ & 0.7 \\
955.750	& 955.900	& 9.2	& $\pm$ & 0.8 \\
955.900	& 956.050	& 9.1	& $\pm$ & 0.7 \\
956.050	& 956.250	& 9.1	& $\pm$ & 0.7 \\
956.250	& 956.400	& 9.1	& $\pm$ & 0.7 \\
956.400	& 956.550	& 9.2	& $\pm$ & 0.8 \\
956.550	& 956.750	& 9.1	& $\pm$ & 0.7 \\
956.750	& 956.900	& 9.2	& $\pm$ & 0.8 \\
956.900	& 957.050	& 9.1	& $\pm$ & 0.7 \\
957.050	& 957.250	& 9.4	& $\pm$ & 0.8 \\
957.250	& 957.400	& 9.3	& $\pm$ & 0.8 \\
957.400	& 957.550	& 9.3	& $\pm$ & 0.8 \\
957.550	& 957.750	& 9.1	& $\pm$ & 0.7 \\
957.750	& 957.900	& 9.1	& $\pm$ & 0.7 \\
957.900	& 958.050	& 9.1	& $\pm$ & 0.7 \\
958.050	& 958.250	& 9.1	& $\pm$ & 0.7 \\
958.250	& 958.400	& 9.1	& $\pm$ & 0.7 \\
958.400	& 958.550	& 9.3	& $\pm$ & 0.8 \\
958.550	& 958.700	& 9.2	& $\pm$ & 0.8 \\
958.700	& 958.900	& 9.2	& $\pm$ & 0.8 \\
958.900	& 962.250	& 9.8	& $\pm$ & 0.8 \\
962.250	& 962.400	& 9.1	& $\pm$ & 0.7 \\
962.400	& 962.600	& 9.2	& $\pm$ & 0.8 \\
962.600	& 962.750	& 9.2	& $\pm$ & 0.8 \\
962.750	& 962.900	& 9.4	& $\pm$ & 0.8 \\
962.900	& 963.050	& 9.2	& $\pm$ & 0.8 \\
963.050	& 963.250	& 9.3	& $\pm$ & 0.8 \\
963.250	& 963.400	& 9.2	& $\pm$ & 0.8 \\
963.400	& 963.550	& 9.2	& $\pm$ & 0.8 \\
963.550	& 963.750	& 9.2	& $\pm$ & 0.8 \\
963.750	& 963.900	& 9.2	& $\pm$ & 0.8 \\
963.900	& 964.050	& 9.2	& $\pm$ & 0.8 \\
964.050	& 964.200	& 9.2	& $\pm$ & 0.8 \\
964.200	& 964.400	& 9.2	& $\pm$ & 0.8 \\
964.400	& 964.550	& 9.2	& $\pm$ & 0.8 \\
964.550	& 964.700	& 9.2	& $\pm$ & 0.8 \\
964.700	& 964.850	& 9.2	& $\pm$ & 0.8 \\
964.850	& 965.050	& 9.2	& $\pm$ & 0.8 \\
965.050	& 965.200	& 9.2	& $\pm$ & 0.8 \\
965.200	& 965.350	& 9.1	& $\pm$ & 0.7 \\
965.350	& 965.550	& 9.2	& $\pm$ & 0.7 \\
965.550	& 965.700	& 9.2	& $\pm$ & 0.8 \\
965.700	& 965.850	& 9.2	& $\pm$ & 0.8 \\
965.850	& 966.000	& 9.2	& $\pm$ & 0.8 \\
966.000	& 966.200	& 9.2	& $\pm$ & 0.8 \\
966.200	& 966.350	& 9.2	& $\pm$ & 0.8 \\
966.350	& 966.500	& 9.2	& $\pm$ & 0.8 \\
966.500	& 966.650	& 9.2	& $\pm$ & 0.8 \\
966.650	& 966.850	& 9.2	& $\pm$ & 0.8 \\
966.850	& 967.000	& 9.2	& $\pm$ & 0.8 \\
967.000	& 967.150	& 9.2	& $\pm$ & 0.8 \\
967.150	& 967.300	& 9.2	& $\pm$ & 0.8 \\
967.300	& 967.500	& 9.2	& $\pm$ & 0.8 \\
967.500	& 967.650	& 9.2	& $\pm$ & 0.8 \\
967.650	& 967.800	& 9.2	& $\pm$ & 0.8 \\
967.800	& 967.950	& 9.2	& $\pm$ & 0.8 \\
967.950	& 968.150	& 9.3	& $\pm$ & 0.8 \\
968.150	& 968.300	& 9.2	& $\pm$ & 0.8 \\
968.300	& 968.450	& 9.2	& $\pm$ & 0.8 \\
968.450	& 968.600	& 9.2	& $\pm$ & 0.8 \\
968.600	& 968.800	& 9.3	& $\pm$ & 0.8 \\
968.800	& 968.950	& 9.2	& $\pm$ & 0.8 \\
968.950	& 969.100	& 9.2	& $\pm$ & 0.8 \\
969.100	& 969.250	& 9.2	& $\pm$ & 0.8 \\
969.250	& 969.400	& 9.2	& $\pm$ & 0.8 \\
969.400	& 969.600	& 9.3	& $\pm$ & 0.8 \\
969.600	& 969.750	& 9.2	& $\pm$ & 0.8 \\
969.750	& 969.900	& 9.2	& $\pm$ & 0.8 \\
969.900	& 970.050	& 9.2	& $\pm$ & 0.8 \\
970.050	& 970.250	& 9.2	& $\pm$ & 0.8 \\
970.250	& 970.400	& 9.2	& $\pm$ & 0.8 \\
970.400	& 970.550	& 9.2	& $\pm$ & 0.8 \\
970.550	& 970.700	& 9.2	& $\pm$ & 0.8 \\
970.700	& 970.900	& 9.2	& $\pm$ & 0.8 \\
970.900	& 971.050	& 9.3	& $\pm$ & 0.8 \\
971.050	& 971.200	& 9.4	& $\pm$ & 0.8 \\
971.200	& 971.350	& 9.2	& $\pm$ & 0.8 \\
971.350	& 971.500	& 9.4	& $\pm$ & 0.8 \\
971.500	& 971.700	& 9.2	& $\pm$ & 0.8 \\
971.700	& 971.850	& 9.3	& $\pm$ & 0.8 \\
971.850	& 972.000	& 9.5	& $\pm$ & 0.8 \\
972.000	& 972.150	& 9.3	& $\pm$ & 0.8 \\
972.150	& 972.350	& 9.3	& $\pm$ & 0.8 \\
972.350	& 972.500	& 9.3	& $\pm$ & 0.8 \\
972.500	& 972.650	& 9.4	& $\pm$ & 0.8 \\
972.650	& 972.800	& 9.6	& $\pm$ & 0.8 \\
972.800	& 973.050	& 9.2	& $\pm$ & 0.8 \\
973.050	& 973.250	& 9.3	& $\pm$ & 0.8 \\
973.250	& 973.400	& 9.3	& $\pm$ & 0.8 \\
973.400	& 973.550	& 9.3	& $\pm$ & 0.8 \\
973.550	& 973.700	& 9.3	& $\pm$ & 0.8 \\
973.700	& 973.850	& 9.3	& $\pm$ & 0.8 \\
973.850	& 974.050	& 9.3	& $\pm$ & 0.8 \\
974.050	& 974.200	& 9.3	& $\pm$ & 0.8 \\
974.200	& 974.350	& 9.3	& $\pm$ & 0.8 \\
974.350	& 974.500	& 9.3	& $\pm$ & 0.8 \\
974.500	& 974.650	& 9.3	& $\pm$ & 0.8 \\
974.650	& 974.850	& 9.3	& $\pm$ & 0.8 \\
974.850	& 975.000	& 9.3	& $\pm$ & 0.8 \\
975.000	& 975.150	& 9.3	& $\pm$ & 0.8 \\
975.150	& 975.300	& 9.3	& $\pm$ & 0.8 \\
975.300	& 975.450	& 9.3	& $\pm$ & 0.8 \\
975.450	& 975.650	& 9.3	& $\pm$ & 0.8 \\
975.650	& 975.800	& 9.3	& $\pm$ & 0.8 \\
975.800	& 975.950	& 9.3	& $\pm$ & 0.8 \\
975.950	& 976.100	& 9.4	& $\pm$ & 0.8 \\
976.100	& 976.250	& 9.3	& $\pm$ & 0.8 \\
976.250	& 976.450	& 9.3	& $\pm$ & 0.8 \\
976.450	& 976.600	& 9.3	& $\pm$ & 0.8 \\
976.600	& 976.750	& 9.3	& $\pm$ & 0.8 \\
976.750	& 976.900	& 9.3	& $\pm$ & 0.8 \\
976.900	& 977.050	& 9.3	& $\pm$ & 0.8 \\
977.050	& 977.250	& 9.4	& $\pm$ & 0.8 \\
977.250	& 977.400	& 9.5	& $\pm$ & 0.8 \\
977.400	& 977.550	& 9.6	& $\pm$ & 0.8 \\
977.550	& 977.700	& 9.5	& $\pm$ & 0.8 \\
977.700	& 977.850	& 9.3	& $\pm$ & 0.8 \\
977.850	& 978.000	& 9.4	& $\pm$ & 0.8 \\
978.000	& 978.200	& 9.4	& $\pm$ & 0.8 \\
978.200	& 978.350	& 9.5	& $\pm$ & 0.8 \\
978.350	& 978.500	& 9.3	& $\pm$ & 0.8 \\
978.500	& 978.650	& 9.3	& $\pm$ & 0.8 \\
978.650	& 978.800	& 9.4	& $\pm$ & 0.8 \\
978.800	& 979.000	& 9.5	& $\pm$ & 0.8 \\
979.000	& 979.150	& 9.3	& $\pm$ & 0.8 \\
979.150	& 979.300	& 9.3	& $\pm$ & 0.8 \\
979.300	& 979.450	& 9.4	& $\pm$ & 0.8 \\
979.450	& 979.600	& 9.3	& $\pm$ & 0.8 \\
979.600	& 979.750	& 9.4	& $\pm$ & 0.8 \\
979.750	& 979.950	& 9.6	& $\pm$ & 0.8 \\
979.950	& 980.100	& 10.3	& $\pm$ & 0.8 \\
980.100	& 980.250	& 10.0	& $\pm$ & 0.8 \\
980.250	& 980.400	& 9.7	& $\pm$ & 0.8 \\
980.400	& 980.550	& 9.5	& $\pm$ & 0.8 \\
980.550	& 980.700	& 9.4	& $\pm$ & 0.8 \\
980.700	& 980.900	& 9.4	& $\pm$ & 0.8 \\
980.900	& 981.050	& 9.4	& $\pm$ & 0.8 \\
981.050	& 981.200	& 9.4	& $\pm$ & 0.8 \\
981.200	& 981.350	& 9.4	& $\pm$ & 0.8 \\
981.350	& 981.500	& 9.5	& $\pm$ & 0.8 \\
981.500	& 981.650	& 9.6	& $\pm$ & 0.8 \\
981.650	& 981.800	& 9.5	& $\pm$ & 0.8 \\
981.800	& 982.100	& 9.4	& $\pm$ & 0.8 \\
982.100	& 982.250	& 9.4	& $\pm$ & 0.8 \\
982.250	& 982.400	& 9.5	& $\pm$ & 0.8 \\
982.400	& 982.550	& 9.5	& $\pm$ & 0.8 \\
982.550	& 982.700	& 9.6	& $\pm$ & 0.8 \\
982.700	& 982.850	& 10.0	& $\pm$ & 0.8 \\
982.850	& 983.050	& 9.6	& $\pm$ & 0.8 \\
983.050	& 983.200	& 9.5	& $\pm$ & 0.8 \\
983.200	& 983.350	& 9.5	& $\pm$ & 0.8 \\
983.350	& 983.500	& 9.5	& $\pm$ & 0.8 \\
983.500	& 983.650	& 9.5	& $\pm$ & 0.8 \\
983.650	& 983.800	& 9.4	& $\pm$ & 0.8 \\
983.800	& 983.950	& 9.4	& $\pm$ & 0.8 \\
983.950	& 984.150	& 9.4	& $\pm$ & 0.8 \\
984.150	& 984.300	& 9.4	& $\pm$ & 0.8 \\
984.300	& 984.450	& 9.4	& $\pm$ & 0.8 \\
984.450	& 984.600	& 9.4	& $\pm$ & 0.8 \\
984.600	& 984.750	& 9.4	& $\pm$ & 0.8 \\
984.750	& 984.900	& 9.4	& $\pm$ & 0.8 \\
984.900	& 985.050	& 9.4	& $\pm$ & 0.8 \\
985.050	& 985.250	& 9.4	& $\pm$ & 0.8 \\
985.250	& 985.400	& 9.6	& $\pm$ & 0.8 \\
985.400	& 985.550	& 9.5	& $\pm$ & 0.8 \\
985.550	& 985.700	& 9.4	& $\pm$ & 0.8 \\
985.700	& 985.850	& 9.5	& $\pm$ & 0.8 \\
985.850	& 986.000	& 9.4	& $\pm$ & 0.8 \\
986.000	& 986.150	& 9.4	& $\pm$ & 0.8 \\
986.150	& 986.300	& 9.4	& $\pm$ & 0.8 \\
986.300	& 986.500	& 9.4	& $\pm$ & 0.8 \\
986.500	& 986.650	& 9.5	& $\pm$ & 0.8 \\
986.650	& 986.800	& 9.5	& $\pm$ & 0.8 \\
986.800	& 986.950	& 9.5	& $\pm$ & 0.8 \\
986.950	& 987.100	& 9.5	& $\pm$ & 0.8 \\
987.100	& 987.250	& 9.5	& $\pm$ & 0.8 \\
987.250	& 987.400	& 9.5	& $\pm$ & 0.8 \\
987.400	& 987.550	& 9.5	& $\pm$ & 0.8 \\
987.550	& 987.750	& 9.5	& $\pm$ & 0.8 \\
987.750	& 987.900	& 9.6	& $\pm$ & 0.8 \\
987.900	& 988.300	& 9.4	& $\pm$ & 0.8 \\
988.300	& 989.150	& 9.6	& $\pm$ & 0.8 \\
989.150	& 989.400	& 9.4	& $\pm$ & 0.8 \\
989.400	& 989.600	& 9.5	& $\pm$ & 0.8 \\
989.600	& 989.750	& 9.4	& $\pm$ & 0.8 \\
989.750	& 989.900	& 9.5	& $\pm$ & 0.8 \\
989.900	& 990.400	& 9.4	& $\pm$ & 0.8 \\
990.400	& 990.650	& 9.4	& $\pm$ & 0.8 \\
990.650	& 990.800	& 9.5	& $\pm$ & 0.8 \\
990.800	& 990.950	& 9.5	& $\pm$ & 0.8 \\
990.950	& 991.100	& 9.8	& $\pm$ & 0.8 \\
991.100	& 991.250	& 10.2	& $\pm$ & 0.8 \\
991.250	& 991.400	& 10.2	& $\pm$ & 0.8 \\
991.400	& 991.550	& 9.6	& $\pm$ & 0.8 \\
991.550	& 991.700	& 9.8	& $\pm$ & 0.8 \\
991.700	& 991.850	& 9.4	& $\pm$ & 0.8 \\
991.850	& 992.000	& 9.4	& $\pm$ & 0.8 \\
992.000	& 992.150	& 9.4	& $\pm$ & 0.8 \\
992.150	& 992.350	& 9.4	& $\pm$ & 0.8 \\
992.350	& 992.500	& 9.4	& $\pm$ & 0.8 \\
992.500	& 992.650	& 9.5	& $\pm$ & 0.8 \\
992.650	& 992.800	& 9.5	& $\pm$ & 0.8 \\
992.800	& 992.950	& 9.5	& $\pm$ & 0.8 \\
992.950	& 993.100	& 9.5	& $\pm$ & 0.8 \\
993.100	& 993.250	& 9.5	& $\pm$ & 0.8 \\
993.250	& 993.400	& 9.4	& $\pm$ & 0.8 \\
993.400	& 993.550	& 9.4	& $\pm$ & 0.8 \\
993.550	& 993.700	& 9.4	& $\pm$ & 0.8 \\
993.700	& 993.850	& 9.4	& $\pm$ & 0.8 \\
993.850	& 994.050	& 9.4	& $\pm$ & 0.8 \\
994.050	& 994.200	& 9.4	& $\pm$ & 0.8 \\
994.200	& 994.350	& 9.4	& $\pm$ & 0.8 \\
994.350	& 994.500	& 9.4	& $\pm$ & 0.8 \\
994.500	& 994.650	& 9.4	& $\pm$ & 0.8 \\
994.650	& 994.800	& 9.4	& $\pm$ & 0.8 \\
994.800	& 994.950	& 9.5	& $\pm$ & 0.8 \\
994.950	& 995.100	& 9.5	& $\pm$ & 0.8 \\
995.100	& 995.250	& 9.5	& $\pm$ & 0.8 \\
995.250	& 995.400	& 9.5	& $\pm$ & 0.8 \\
995.400	& 995.550	& 9.5	& $\pm$ & 0.8 \\
995.550	& 995.700	& 9.5	& $\pm$ & 0.8 \\
995.700	& 995.850	& 9.5	& $\pm$ & 0.8 \\
995.850	& 996.050	& 9.8	& $\pm$ & 0.8 \\
996.050	& 996.200	& 9.7	& $\pm$ & 0.8 \\
996.200	& 996.350	& 9.7	& $\pm$ & 0.8 \\
996.350	& 996.500	& 9.6	& $\pm$ & 0.8 \\
996.500	& 996.650	& 9.4	& $\pm$ & 0.8 \\
996.650	& 996.800	& 9.4	& $\pm$ & 0.8 \\
996.800	& 996.950	& 9.4	& $\pm$ & 0.8 \\
996.950	& 997.100	& 9.4	& $\pm$ & 0.8 \\
997.100	& 997.250	& 9.4	& $\pm$ & 0.8 \\
997.250	& 997.400	& 9.4	& $\pm$ & 0.8 \\
997.400	& 997.550	& 9.4	& $\pm$ & 0.8 \\
997.550	& 997.700	& 9.4	& $\pm$ & 0.8 \\
997.700	& 997.850	& 9.4	& $\pm$ & 0.8 \\
997.850	& 998.000	& 9.4	& $\pm$ & 0.8 \\
998.000	& 998.150	& 9.4	& $\pm$ & 0.8 \\
998.150	& 998.300	& 9.4	& $\pm$ & 0.8 \\
998.300	& 998.500	& 9.4	& $\pm$ & 0.8 \\
998.500	& 998.650	& 9.5	& $\pm$ & 0.8 \\
998.650	& 998.800	& 9.4	& $\pm$ & 0.8 \\
998.800	& 998.950	& 9.4	& $\pm$ & 0.8 \\
998.950	& 999.100	& 9.4	& $\pm$ & 0.8 \\
999.100	& 999.250	& 9.4	& $\pm$ & 0.8 \\
999.250	& 999.400	& 9.4	& $\pm$ & 0.8 \\
999.400	& 999.550	& 9.4	& $\pm$ & 0.8 \\
999.550	& 999.700	& 9.4	& $\pm$ & 0.8 \\
999.700	& 999.850	& 9.5	& $\pm$ & 0.8 \\
\hline
\hline
\caption{We divided the frequency range into 2000 partitions of approximately
equal search volume. The first two columns list the start and stop
frequency of each partition in Hz. The second two columns list the
90\% upper limits on the gravitational wave strain $h_0^{90\%}$ and
the 1-$\sigma$ uncertainty on $h_0^{90\%}$.
}\label{table_UL}
\end{longtable}


==> table_excluded.tex <==
\begin{longtable}{|rr|}
\hline
\hline
\textbf{start} & \textbf{stop} \\ 
\textbf{band} & \textbf{band} \\ 
\hline
\hline
\endhead
50.100	&   \\
51.100	&   \\
51.950	& 52.000 \\
52.450	&   \\
52.900	& 53.100 \\
53.900	&   \\
54.400	& 54.750 \\
55.050	& 55.100 \\
55.450	& 55.500 \\
55.600	&   \\
55.700	& 55.900 \\
56.100	& 56.500 \\
56.750	&   \\
58.350	& 58.400 \\
58.500	& 58.600 \\
58.700	& 60.950 \\
61.050	&   \\
61.300	& 61.450 \\
62.250	& 62.300 \\
63.150	&   \\
63.450	& 63.500 \\
63.950	& 64.100 \\
64.300	& 64.500 \\
64.750	& 64.850 \\
65.350	& 65.400 \\
68.500	&   \\
68.800	& 68.950 \\
69.650	& 69.750 \\
70.050	& 70.150 \\
70.500	&   \\
72.350	& 72.450 \\
72.900	& 73.050 \\
73.300	& 73.450 \\
73.800	&   \\
73.900	&   \\
74.500	& 74.550 \\
76.050	&   \\
77.600	& 77.700 \\
78.200	& 78.600 \\
79.950	& 80.050 \\
80.400	&   \\
80.550	& 80.650 \\
81.100	& 81.200 \\
83.450	&   \\
83.950	& 84.000 \\
85.650	& 85.800 \\
86.700	& 86.850 \\
89.950	& 90.000 \\
90.700	& 90.750 \\
92.100	&   \\
93.100	&   \\
93.850	& 94.000 \\
94.200	&   \\
95.950	& 96.100 \\
96.700	& 97.200 \\
98.950	& 99.050 \\
99.900	& 100.100 \\
101.950	& 102.000 \\
103.100	&   \\
103.950	&   \\
104.900	&   \\
106.450	& 106.500 \\
106.650	&   \\
107.100	& 107.150 \\
107.300	&   \\
107.400	&   \\
107.950	& 108.150 \\
108.750	& 109.100 \\
110.600	&   \\
111.000	& 111.100 \\
111.750	& 112.100 \\
113.200	& 113.300 \\
113.700	& 113.850 \\
114.650	& 114.700 \\
115.250	& 115.400 \\
117.500	& 117.550 \\
117.650	&   \\
118.250	& 118.300 \\
118.850	&   \\
119.250	&   \\
119.400	&   \\
119.800	& 120.200 \\
121.050	&   \\
121.150	& 121.300 \\
121.600	&   \\
121.700	&   \\
121.950	& 122.100 \\
122.550	&   \\
126.750	&   \\
127.050	&   \\
127.950	& 128.100 \\
129.650	& 129.750 \\
129.900	&   \\
131.950	&   \\
132.700	& 132.750 \\
135.100	&   \\
137.100	&   \\
137.450	& 137.950 \\
139.450	& 139.650 \\
139.950	& 140.050 \\
140.150	& 140.400 \\
141.600	& 141.650 \\
141.950	&   \\
142.150	&   \\
143.950	& 144.100 \\
144.800	& 145.850 \\
146.650	& 146.950 \\
147.950	&   \\
149.800	& 150.050 \\
157.950	& 158.000 \\
159.950	& 160.000 \\
163.450	& 163.650 \\
165.950	&   \\
166.100	&   \\
167.950	& 168.100 \\
172.950	&   \\
175.950	& 176.100 \\
179.100	&   \\
179.400	& 179.500 \\
179.600	& 180.300 \\
180.400	&   \\
180.850	&   \\
181.250	&   \\
182.800	&   \\
183.950	&   \\
184.400	&   \\
185.400	&   \\
185.950	&   \\
187.950	&   \\
188.450	&   \\
189.350	&   \\
191.800	&   \\
191.950	& 192.000 \\
192.350	& 192.550 \\
193.500	&   \\
193.650	& 194.300 \\
195.950	& 196.050 \\
196.950	& 197.000 \\
197.700	& 197.950 \\
198.150	&   \\
198.550	&   \\
199.150	& 199.400 \\
199.750	&   \\
199.850	&   \\
199.950	& 200.000 \\
205.750	& 206.100 \\
206.450	& 206.850 \\
209.250	&   \\
210.250	& 210.450 \\
213.950	&   \\
215.950	&   \\
217.300	& 217.750 \\
217.950	& 218.000 \\
221.950	&   \\
223.950	& 224.000 \\
225.550	&   \\
228.950	&   \\
229.850	&   \\
230.200	& 230.250 \\
231.350	&   \\
233.700	& 234.100 \\
239.700	& 240.050 \\
240.150	&   \\
242.150	& 242.900 \\
243.000	& 243.400 \\
243.950	& 244.000 \\
249.950	&   \\
251.750	& 252.100 \\
255.950	& 256.000 \\
261.700	& 262.300 \\
263.950	&   \\
268.800	& 268.950 \\
269.950	&   \\
275.300	& 275.850 \\
277.950	&   \\
279.950	&   \\
281.950	&   \\
289.650	& 290.300 \\
291.000	&   \\
291.350	&   \\
294.650	&   \\
299.550	& 299.850 \\
299.950	& 300.000 \\
300.100	& 300.200 \\
300.350	&   \\
305.950	&   \\
306.500	&   \\
307.950	& 308.000 \\
308.500	&   \\
317.650	& 318.350 \\
320.350	&   \\
324.000	&   \\
328.850	& 330.150 \\
332.200	&   \\
335.400	& 335.800 \\
338.650	&   \\
338.750	& 338.800 \\
339.050	& 339.100 \\
339.500	&   \\
339.650	& 339.800 \\
339.950	&   \\
340.050	& 340.100 \\
340.400	&   \\
340.650	& 340.700 \\
340.950	& 341.000 \\
342.600	&   \\
342.800	& 342.950 \\
343.050	& 344.850 \\
345.000	& 345.100 \\
345.200	&   \\
345.950	& 346.000 \\
346.250	& 347.900 \\
348.050	&   \\
348.550	&   \\
348.700	&   \\
349.800	&   \\
350.050	& 350.200 \\
350.350	& 350.600 \\
350.700	& 350.750 \\
350.950	& 351.100 \\
351.350	& 351.500 \\
355.800	& 356.050 \\
357.900	&   \\
359.600	&   \\
359.950	&   \\
366.550	&   \\
369.650	& 370.500 \\
371.750	&   \\
373.550	& 374.150 \\
383.500	& 383.650 \\
389.550	& 389.650 \\
389.750	&   \\
391.250	&   \\
391.800	& 392.350 \\
392.650	& 394.300 \\
394.850	&   \\
396.250	& 397.150 \\
397.300	&   \\
397.400	& 397.500 \\
399.050	&   \\
399.250	& 399.300 \\
399.750	& 400.850 \\
401.050	& 401.150 \\
401.250	&   \\
401.950	& 402.000 \\
403.300	& 404.250 \\
406.950	&   \\
407.250	& 407.300 \\
408.250	&   \\
409.300	& 409.350 \\
411.950	& 412.000 \\
413.050	& 413.700 \\
416.150	& 416.200 \\
416.600	& 417.550 \\
417.950	&   \\
418.150	&   \\
423.150	& 423.200 \\
429.500	&   \\
429.650	& 430.150 \\
434.600	& 435.250 \\
439.600	&   \\
439.700	& 440.150 \\
440.950	& 441.000 \\
444.450	& 444.650 \\
451.450	& 451.800 \\
454.950	& 455.000 \\
457.950	& 458.000 \\
460.600	& 460.800 \\
467.700	& 468.200 \\
472.600	&   \\
481.900	& 482.450 \\
485.950	& 486.950 \\
490.950	&   \\
495.950	& 496.100 \\
512.150	& 512.200 \\
515.950	&   \\
518.600	&   \\
523.400	& 524.200 \\
531.950	&   \\
545.550	&   \\
545.700	& 546.200 \\
550.800	& 552.250 \\
561.950	&   \\
563.550	& 564.300 \\
565.750	& 566.250 \\
567.450	& 568.550 \\
569.950	& 570.000 \\
575.050	& 575.150 \\
579.350	& 580.550 \\
589.300	&   \\
601.150	&   \\
607.400	& 608.250 \\
615.000	&   \\
626.850	& 626.900 \\
635.250	& 636.250 \\
645.350	& 645.400 \\
645.600	& 646.800 \\
646.900	& 647.100 \\
648.050	& 648.850 \\
648.950	&   \\
649.350	&   \\
652.550	& 652.650 \\
658.050	& 660.000 \\
663.900	& 664.050 \\
666.400	& 666.450 \\
685.700	&   \\
686.050	& 689.500 \\
689.600	& 690.350 \\
690.450	& 690.600 \\
691.650	& 692.250 \\
692.500	&   \\
692.900	& 694.950 \\
695.050	& 695.200 \\
695.350	& 695.450 \\
695.550	&   \\
695.800	&   \\
695.950	&   \\
703.250	& 704.400 \\
704.500	&   \\
729.150	& 729.850 \\
729.950	& 730.000 \\
755.400	&   \\
757.550	&   \\
757.800	&   \\
757.950	&   \\
767.250	&   \\
785.950	&   \\
792.950	& 793.000 \\
796.400	& 797.750 \\
799.400	& 800.250 \\
800.400	& 801.550 \\
803.950	&   \\
806.800	& 806.850 \\
813.950	& 814.050 \\
826.400	&   \\
832.550	&   \\
841.950	& 842.050 \\
844.400	& 844.450 \\
869.000	& 870.950 \\
871.100	& 871.200 \\
895.550	& 895.900 \\
897.200	& 898.400 \\
920.550	& 922.350 \\
924.400	& 924.450 \\
925.350	&   \\
925.450	& 926.400 \\
927.900	& 928.250 \\
931.400	& 931.450 \\
951.000	& 951.050 \\
951.150	& 951.200 \\
951.300	& 951.350 \\
951.500	&   \\
951.600	&   \\
951.700	&   \\
953.900	& 954.250 \\
958.950	& 962.100 \\
972.950	& 973.000 \\
981.900	& 981.950 \\
987.950	& 988.100 \\
988.250	&   \\
988.350	& 988.950 \\
989.050	&   \\
989.250	&   \\
989.350	&   \\
989.450	&   \\
989.950	& 990.250 \\
990.550	&   \\
999.900	& 999.950 \\
\hline
\hline
\caption{This table lists the 50-mHz search bands that contain
non-Gaussian disturbances and are therefore excluded
from the search. The first and second columns list the
start frequencies of the first and last 50-mHz band of
a contiguous range of excluded bands. We do not perform
any up-front line cleaning in this search.}
\label{table_excluded}
\end{longtable}



